Speech Robust Bench: A Robustness Benchmark For Speech Recognition

As Automatic Speech Recognition (ASR) models become ever more pervasive, it is important to ensure that they make reliable predictions under corruptions present in the physical and digital world. We propose Speech Robust Bench (SRB), a comprehensive benchmark for evaluating the robustness of ASR models to diverse corruptions. SRB is composed of 114 input perturbations which simulate an heterogeneous range of corruptions that ASR models may encounter when deployed in the wild. We use SRB to evaluate the robustness of several state-of-the-art ASR models and observe that model size and certain modeling choices such as the use of discrete representations, or self-training appear to be conducive to robustness. We extend this analysis to measure the robustness of ASR models on data from various demographic subgroups, namely English and Spanish speakers, and males and females. Our results revealed noticeable disparities in the model's robustness across subgroups. We believe that SRB will significantly facilitate future research towards robust ASR models, by making it easier to conduct comprehensive and comparable robustness evaluations.

==> texfiles/acks.tex <==
The execution of this work was funded by the European Union’s Horizon 2020 RIA SPATIAL project (Grant Agreement No. 101021808), RIA ELOQUENCE project (Grant Agreement No. 101135916) and from the Spanish Project 6G-RIEMANN (Grant Agreement No. 2022/0005420). The authors bear the sole responsibility for the content presented in this paper, and any interpretations or conclusions drawn from it do not reflect the official position of the funding agencies.

==> texfiles/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:limitations}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We do not believe there are any. In fact, we belive that by facilitating robustness evaluation, we will make a positive impact.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}{see Introduction}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{see Section 3, and Table \ref{sec:perturbs}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{see appendix}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}{}
  \item Did you mention the license of the assets?
    \answerYes{see \S\ref{sec:license}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}

==> texfiles/noise_dataset_table.tex <==
\begin{tabular}{r c c}
    \toprule
    name & hours & recordings \\
    \midrule
    ESC-50 & 2.78 & 2000 \\
    MUSAN & 108.5 & 2016 \\
    WHAM! & 9 & 3000 \\
    MS-SNSD & 0.7 & 51 \\
    \bottomrule
\end{tabular}

==> texfiles/relatex_table.tex <==

\begin{table}
    \centering
    \begin{tabular}{cccccccc}
          & Accent & Synth. Speech & Env. Noise & Spatial &  &  & \\
         CHiME-6~\citep{barker2017chime} &  &  &  &  &  &  & \\
         &  &  &  &  &  &  & \\
         &  &  &  &  &  &  & \\
         &  &  &  &  &  &  & \\
         &  &  &  &  &  &  & \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> texfiles/table_full_results.tex <==
\begin{tabular}{lllrrrr}
 &  &  & NWER & NWERD & WER & WERD \\
model (abrv) & dataset & augmentation &  &  &  &  \\
\multirow[c]{85}{*}{cnry-1b} & \multirow[c]{25}{*}{LibriSpeech} & clean & 0.13 & 0.00 & 1.70 & 0.00 \\
 &  & crosstalk & 0.23 & 0.18 & 12.59 & 10.89 \\
 &  & echo & 0.26 & 0.23 & 13.09 & 11.38 \\
 &  & env noise & 0.06 & 0.04 & 4.92 & 3.22 \\
 &  & env noise esc50 & 0.04 & 0.01 & 2.22 & 0.52 \\
 &  & env noise musan & 0.05 & 0.01 & 2.53 & 0.83 \\
 &  & env noise wham & 0.06 & 0.02 & 3.40 & 1.70 \\
 &  & gain & 0.03 & 0.01 & 2.22 & 0.52 \\
 &  & gnoise & 0.05 & 0.03 & 4.37 & 2.66 \\
 &  & highpass & 0.42 & 0.39 & 30.33 & 28.62 \\
 &  & lowpass & 0.20 & 0.16 & 14.43 & 12.72 \\
 &  & music & 0.05 & 0.01 & 2.63 & 0.93 \\
 &  & pgd & 0.90 & 0.87 & 63.44 & 61.73 \\
 &  & phaser & 0.15 & 0.09 & 8.38 & 6.68 \\
 &  & pitch down & 0.29 & 0.26 & 23.72 & 22.01 \\
 &  & pitch up & 0.20 & 0.17 & 12.67 & 10.96 \\
 &  & real rir & 0.22 & 0.19 & 17.01 & 15.31 \\
 &  & resample & 0.17 & 0.11 & 8.89 & 7.19 \\
 &  & rir & 0.04 & 0.02 & 3.00 & 1.30 \\
 &  & slowdown & 0.27 & 0.25 & 20.31 & 18.61 \\
 &  & speedup & 0.44 & 0.41 & 30.23 & 28.53 \\
 &  & tempo down & 0.04 & 0.00 & 1.96 & 0.26 \\
 &  & tempo up & 0.05 & 0.02 & 3.25 & 1.55 \\
 &  & universal adv & 9.00 & 7.68 & 9.38 & 7.68 \\
 &  & voice conversion & 0.12 & 0.09 & 5.95 & 4.24 \\
 & \multirow[c]{27}{*}{MLS-ES} & bass & 0.51 & 0.40 & 15.64 & 12.43 \\
 &  & chorus & 0.44 & 0.32 & 15.49 & 12.27 \\
 &  & clean & 0.14 & 0.00 & 3.21 & 0.00 \\
 &  & crosstalk & 0.76 & 0.60 & 20.20 & 16.98 \\
 &  & echo & 0.80 & 0.68 & 21.58 & 18.37 \\
 &  & env noise & 0.37 & 0.32 & 32.01 & 28.79 \\
 &  & env noise esc50 & 0.19 & 0.03 & 4.55 & 1.34 \\
 &  & env noise musan & 0.15 & 0.04 & 5.50 & 2.29 \\
 &  & env noise wham & 0.17 & 0.06 & 8.97 & 5.76 \\
 &  & gain & 0.22 & 0.16 & 12.34 & 9.12 \\
 &  & gnoise & 0.13 & 0.08 & 11.46 & 8.24 \\
 &  & highpass & 0.59 & 0.51 & 39.97 & 36.75 \\
 &  & lowpass & 0.22 & 0.16 & 17.75 & 14.54 \\
 &  & music & 0.13 & 0.04 & 5.75 & 2.53 \\
 &  & pgd & 1.44 & 1.38 & 87.51 & 84.30 \\
 &  & phaser & 0.43 & 0.29 & 23.49 & 20.27 \\
 &  & pitch down & 0.49 & 0.42 & 34.42 & 31.21 \\
 &  & pitch up & 0.77 & 0.66 & 28.62 & 25.40 \\
 &  & resample & 0.19 & 0.07 & 8.20 & 4.99 \\
 &  & rir & 0.16 & 0.08 & 6.60 & 3.39 \\
 &  & slowdown & 0.58 & 0.43 & 30.29 & 27.09 \\
 &  & speedup & 0.95 & 0.82 & 45.28 & 42.06 \\
 &  & tempo down & 0.27 & 0.02 & 3.64 & 0.43 \\
 &  & tempo up & 0.24 & 0.10 & 7.62 & 4.41 \\
 &  & treble & 0.22 & 0.00 & 3.28 & 0.07 \\
 &  & tremolo & 0.12 & 0.01 & 3.53 & 0.32 \\
 &  & universal adv & 0.62 & 0.51 & 29.27 & 26.05 \\
 & \multirow[c]{28}{*}{TEDLIUM} & bass & 0.34 & 0.01 & 10.62 & 0.37 \\
 &  & chorus & 0.21 & 0.05 & 13.48 & 3.23 \\
 &  & clean & 0.31 & 0.00 & 10.25 & 0.00 \\
 &  & crosstalk & 0.41 & 0.17 & 21.23 & 10.98 \\
 &  & echo & 0.41 & 0.23 & 23.86 & 13.61 \\
 &  & env noise & 0.25 & 0.04 & 13.38 & 3.13 \\
 &  & env noise esc50 & 0.21 & 0.01 & 10.99 & 0.74 \\
 &  & env noise musan & 0.23 & 0.01 & 11.29 & 1.04 \\
 &  & env noise wham & 0.24 & 0.02 & 12.13 & 1.88 \\
 &  & gain & 0.15 & 0.03 & 12.48 & 2.23 \\
 &  & gnoise & 0.15 & 0.03 & 13.18 & 2.93 \\
 &  & highpass & 0.61 & 0.45 & 46.41 & 36.16 \\
 &  & lowpass & 0.37 & 0.15 & 21.63 & 11.45 \\
 &  & music & 0.24 & 0.01 & 11.25 & 1.00 \\
 &  & phaser & 0.40 & 0.16 & 22.92 & 12.67 \\
 &  & pitch down & 0.46 & 0.32 & 36.60 & 26.35 \\
 &  & pitch up & 0.34 & 0.19 & 24.17 & 13.92 \\
 &  & real rir & 0.42 & 0.24 & 30.25 & 20.00 \\
 &  & resample & 0.45 & 0.18 & 21.40 & 11.27 \\
 &  & rir & 0.16 & 0.02 & 11.87 & 1.62 \\
 &  & slowdown & 0.47 & 0.32 & 34.87 & 24.66 \\
 &  & speedup & 0.56 & 0.40 & 40.28 & 30.03 \\
 &  & tempo down & 0.17 & 0.01 & 10.81 & 0.56 \\
 &  & tempo up & 0.20 & 0.05 & 13.83 & 3.58 \\
 &  & treble & 0.30 & 0.00 & 10.35 & 0.10 \\
 &  & tremolo & 0.26 & 0.02 & 11.02 & 0.77 \\
 &  & universal adv & 0.56 & 0.30 & 32.14 & 21.89 \\
 &  & voice conversion & 0.23 & 0.03 & 11.73 & 1.48 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.40 & 0.38 & 33.42 & 31.71 \\
 &  & itw nf ami & 0.44 & 0.39 & 15.62 & 13.92 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.57 & 0.56 & 57.30 & 55.60 \\
 &  & itw nf & 0.39 & 0.37 & 30.54 & 28.83 \\
 & common voice & accent & 0.39 & 0.28 & 6.30 & 4.60 \\
\multirow[c]{60}{*}{ds} & \multirow[c]{28}{*}{LibriSpeech} & bass & 0.93 & 0.27 & 26.40 & 11.34 \\
 &  & chorus & 1.09 & 0.81 & 61.50 & 46.45 \\
 &  & clean & 1.12 & 0.00 & 15.05 & 0.00 \\
 &  & crosstalk & 1.06 & 0.65 & 50.84 & 35.79 \\
 &  & echo & 1.49 & 1.20 & 76.98 & 61.93 \\
 &  & env noise & 0.55 & 0.31 & 40.00 & 24.95 \\
 &  & env noise esc50 & 0.93 & 0.64 & 53.61 & 38.56 \\
 &  & env noise musan & 0.60 & 0.25 & 32.02 & 17.20 \\
 &  & env noise wham & 0.62 & 0.27 & 37.29 & 22.24 \\
 &  & gain & 0.69 & 0.46 & 47.02 & 31.97 \\
 &  & gnoise & 0.47 & 0.29 & 43.97 & 28.94 \\
 &  & highpass & 1.11 & 0.83 & 67.03 & 51.98 \\
 &  & lowpass & 0.93 & 0.61 & 53.14 & 38.09 \\
 &  & music & 0.62 & 0.26 & 33.53 & 18.48 \\
 &  & pgd & 1.19 & 0.90 & 78.00 & 62.95 \\
 &  & phaser & 1.02 & 0.49 & 41.73 & 26.68 \\
 &  & pitch down & 1.01 & 0.80 & 75.32 & 60.27 \\
 &  & pitch up & 1.16 & 0.91 & 70.90 & 55.85 \\
 &  & real rir & 1.02 & 0.74 & 68.66 & 53.61 \\
 &  & resample & 1.05 & 0.51 & 44.43 & 29.38 \\
 &  & rir & 0.55 & 0.32 & 37.98 & 22.93 \\
 &  & slowdown & 0.97 & 0.71 & 62.38 & 47.33 \\
 &  & speedup & 1.18 & 0.93 & 74.91 & 59.86 \\
 &  & tempo down & 0.41 & 0.12 & 21.26 & 6.21 \\
 &  & tempo up & 0.66 & 0.40 & 40.54 & 25.49 \\
 &  & treble & 0.71 & 0.02 & 15.01 & 1.27 \\
 &  & tremolo & 0.75 & 0.21 & 26.32 & 11.26 \\
 &  & voice conversion & 0.67 & 0.37 & 33.09 & 18.04 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 1.40 & 0.16 & 46.25 & 8.24 \\
 &  & chorus & 1.14 & 0.53 & 72.24 & 34.23 \\
 &  & clean & 1.14 & 0.00 & 38.01 & 0.00 \\
 &  & crosstalk & 1.31 & 0.41 & 62.96 & 24.95 \\
 &  & echo & 1.54 & 0.90 & 91.05 & 53.04 \\
 &  & env noise & 1.03 & 0.23 & 55.49 & 17.56 \\
 &  & env noise esc50 & 0.87 & 0.14 & 48.26 & 10.25 \\
 &  & env noise musan & 1.00 & 0.20 & 52.28 & 14.27 \\
 &  & env noise wham & 0.99 & 0.19 & 54.59 & 16.59 \\
 &  & gain & 1.01 & 0.56 & 85.46 & 47.45 \\
 &  & gnoise & 0.70 & 0.25 & 62.29 & 24.28 \\
 &  & highpass & 1.27 & 0.66 & 83.39 & 45.38 \\
 &  & lowpass & 1.49 & 0.68 & 74.98 & 36.97 \\
 &  & music & 1.00 & 0.17 & 50.56 & 12.76 \\
 &  & pgd & 1.20 & 0.65 & 89.49 & 51.48 \\
 &  & phaser & 1.45 & 0.55 & 69.28 & 31.27 \\
 &  & pitch down & 1.19 & 0.68 & 89.65 & 51.64 \\
 &  & pitch up & 1.24 & 0.69 & 86.41 & 48.40 \\
 &  & real rir & 1.24 & 0.60 & 84.36 & 46.35 \\
 &  & resample & 1.65 & 0.63 & 68.77 & 30.76 \\
 &  & rir & 1.16 & 0.63 & 84.78 & 46.77 \\
 &  & slowdown & 1.21 & 0.64 & 83.17 & 45.16 \\
 &  & speedup & 1.28 & 0.71 & 87.70 & 49.69 \\
 &  & tempo down & 0.79 & 0.19 & 50.81 & 12.81 \\
 &  & tempo up & 1.02 & 0.45 & 69.11 & 31.10 \\
 &  & treble & 1.20 & 0.09 & 43.34 & 5.37 \\
 &  & tremolo & 1.13 & 0.22 & 50.53 & 12.52 \\
 &  & universal adv & 1.18 & 0.23 & 52.97 & 15.27 \\
 &  & voice conversion & 0.91 & 0.15 & 45.29 & 7.28 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 1.06 & 0.90 & 105.60 & 90.55 \\
 &  & itw nf & 1.27 & 1.07 & 99.01 & 83.96 \\
 & common voice & accent & 5.33 & 4.41 & 108.41 & 93.36 \\
\multirow[c]{63}{*}{hubt-lg} & \multirow[c]{29}{*}{LibriSpeech} & bass & 0.11 & 0.02 & 3.29 & 1.21 \\
 &  & chorus & 0.18 & 0.14 & 10.45 & 8.37 \\
 &  & clean & 0.15 & 0.00 & 2.08 & 0.00 \\
 &  & crosstalk & 0.47 & 0.42 & 25.42 & 23.34 \\
 &  & echo & 0.67 & 0.63 & 34.48 & 32.40 \\
 &  & env noise & 0.12 & 0.08 & 9.34 & 7.25 \\
 &  & env noise esc50 & 0.20 & 0.16 & 13.67 & 11.59 \\
 &  & env noise musan & 0.09 & 0.04 & 4.86 & 2.79 \\
 &  & env noise wham & 0.11 & 0.06 & 7.30 & 5.22 \\
 &  & gain & 0.05 & 0.01 & 3.14 & 1.05 \\
 &  & gnoise & 0.11 & 0.09 & 11.16 & 9.07 \\
 &  & highpass & 0.43 & 0.39 & 29.73 & 27.65 \\
 &  & lowpass & 0.22 & 0.17 & 15.80 & 13.72 \\
 &  & music & 0.10 & 0.05 & 6.00 & 3.92 \\
 &  & pgd & 0.75 & 0.71 & 52.11 & 50.02 \\
 &  & phaser & 0.11 & 0.04 & 4.82 & 2.74 \\
 &  & pitch down & 0.43 & 0.40 & 34.53 & 32.45 \\
 &  & pitch up & 0.48 & 0.44 & 29.84 & 27.75 \\
 &  & real rir & 0.19 & 0.15 & 13.83 & 11.75 \\
 &  & resample & 0.13 & 0.06 & 5.91 & 3.83 \\
 &  & rir & 0.04 & 0.01 & 2.86 & 0.78 \\
 &  & slowdown & 0.32 & 0.28 & 22.94 & 20.86 \\
 &  & speedup & 0.54 & 0.50 & 36.93 & 34.85 \\
 &  & tempo down & 0.04 & 0.00 & 2.22 & 0.14 \\
 &  & tempo up & 0.14 & 0.11 & 9.11 & 7.03 \\
 &  & treble & 0.11 & 0.00 & 2.08 & 0.01 \\
 &  & tremolo & 0.08 & 0.00 & 2.15 & 0.07 \\
 &  & universal adv & 36.49 & 34.88 & 36.96 & 34.88 \\
 &  & voice conversion & 0.18 & 0.13 & 8.62 & 6.54 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.49 & 0.01 & 15.51 & 0.81 \\
 &  & chorus & 0.43 & 0.20 & 27.91 & 13.20 \\
 &  & clean & 0.44 & 0.00 & 14.71 & 0.00 \\
 &  & crosstalk & 0.68 & 0.33 & 35.75 & 21.04 \\
 &  & echo & 0.75 & 0.50 & 44.48 & 29.77 \\
 &  & env noise & 0.41 & 0.10 & 23.25 & 8.54 \\
 &  & env noise esc50 & 0.40 & 0.12 & 23.75 & 9.04 \\
 &  & env noise musan & 0.36 & 0.05 & 18.68 & 3.98 \\
 &  & env noise wham & 0.39 & 0.08 & 21.89 & 7.18 \\
 &  & gain & 0.33 & 0.15 & 28.33 & 13.62 \\
 &  & gnoise & 0.29 & 0.12 & 26.78 & 12.08 \\
 &  & highpass & 0.72 & 0.48 & 51.69 & 36.98 \\
 &  & lowpass & 0.60 & 0.28 & 34.49 & 19.78 \\
 &  & music & 0.39 & 0.06 & 19.83 & 5.13 \\
 &  & pgd & 0.38 & 0.17 & 28.56 & 13.85 \\
 &  & phaser & 0.47 & 0.12 & 24.32 & 9.61 \\
 &  & pitch down & 0.68 & 0.48 & 52.74 & 38.03 \\
 &  & pitch up & 0.64 & 0.42 & 45.19 & 30.48 \\
 &  & real rir & 0.43 & 0.19 & 29.28 & 14.57 \\
 &  & resample & 0.55 & 0.16 & 24.11 & 9.41 \\
 &  & rir & 0.31 & 0.11 & 22.73 & 8.02 \\
 &  & slowdown & 0.54 & 0.32 & 38.62 & 23.94 \\
 &  & speedup & 0.79 & 0.57 & 56.41 & 41.70 \\
 &  & tempo down & 0.24 & 0.01 & 15.06 & 0.41 \\
 &  & tempo up & 0.49 & 0.27 & 33.81 & 19.10 \\
 &  & treble & 0.43 & 0.00 & 14.89 & 0.20 \\
 &  & tremolo & 0.36 & 0.01 & 15.40 & 0.69 \\
 &  & universal adv & 0.38 & 0.01 & 15.39 & 0.68 \\
 &  & voice conversion & 0.48 & 0.18 & 23.82 & 9.11 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.63 & 0.61 & 53.05 & 50.97 \\
 &  & itw nf ami & 0.83 & 0.78 & 29.82 & 27.74 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.84 & 0.82 & 84.19 & 82.11 \\
 &  & itw nf & 0.73 & 0.71 & 57.33 & 55.25 \\
 & common voice & accent & 0.97 & 0.85 & 16.17 & 14.08 \\
\multirow[c]{62}{*}{hubt-xl} & \multirow[c]{28}{*}{LibriSpeech} & bass & 0.12 & 0.01 & 2.32 & 0.27 \\
 &  & clean & 0.15 & 0.00 & 2.05 & 0.00 \\
 &  & crosstalk & 0.48 & 0.43 & 26.16 & 24.11 \\
 &  & echo & 0.65 & 0.61 & 33.23 & 31.18 \\
 &  & env noise & 0.14 & 0.10 & 11.01 & 8.95 \\
 &  & env noise esc50 & 0.25 & 0.21 & 17.01 & 14.96 \\
 &  & env noise musan & 0.11 & 0.06 & 6.35 & 4.29 \\
 &  & env noise wham & 0.15 & 0.10 & 10.70 & 8.65 \\
 &  & gain & 0.07 & 0.04 & 4.70 & 2.65 \\
 &  & gnoise & 0.18 & 0.16 & 18.39 & 16.34 \\
 &  & highpass & 0.71 & 0.67 & 47.46 & 45.40 \\
 &  & lowpass & 0.29 & 0.25 & 21.29 & 19.23 \\
 &  & music & 0.12 & 0.07 & 7.52 & 5.47 \\
 &  & pgd & 0.83 & 0.79 & 56.42 & 54.37 \\
 &  & phaser & 0.10 & 0.03 & 4.28 & 2.23 \\
 &  & pitch down & 0.48 & 0.45 & 38.51 & 36.46 \\
 &  & pitch up & 0.48 & 0.45 & 30.18 & 28.12 \\
 &  & real rir & 0.20 & 0.16 & 14.24 & 12.18 \\
 &  & resample & 0.16 & 0.09 & 7.52 & 5.46 \\
 &  & rir & 0.04 & 0.01 & 2.94 & 0.88 \\
 &  & slowdown & 0.38 & 0.35 & 27.39 & 25.34 \\
 &  & speedup & 0.57 & 0.54 & 39.12 & 37.07 \\
 &  & tempo down & 0.05 & 0.01 & 2.42 & 0.36 \\
 &  & tempo up & 0.15 & 0.11 & 9.58 & 7.53 \\
 &  & treble & 0.11 & 0.00 & 2.10 & 0.05 \\
 &  & tremolo & 0.08 & 0.01 & 2.40 & 0.35 \\
 &  & universal adv & 28.28 & 26.69 & 28.76 & 26.70 \\
 &  & voice conversion & 0.15 & 0.11 & 7.51 & 5.46 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.50 & 0.02 & 15.64 & 0.92 \\
 &  & chorus & 0.43 & 0.19 & 27.47 & 12.75 \\
 &  & clean & 0.44 & 0.00 & 14.72 & 0.00 \\
 &  & crosstalk & 0.69 & 0.34 & 36.52 & 21.79 \\
 &  & echo & 0.76 & 0.51 & 44.99 & 30.27 \\
 &  & env noise & 0.43 & 0.12 & 24.58 & 9.85 \\
 &  & env noise esc50 & 0.47 & 0.19 & 28.22 & 13.50 \\
 &  & env noise musan & 0.38 & 0.07 & 19.95 & 5.23 \\
 &  & env noise wham & 0.41 & 0.11 & 24.51 & 9.79 \\
 &  & gain & 0.39 & 0.21 & 33.46 & 18.74 \\
 &  & gnoise & 0.35 & 0.17 & 31.99 & 17.29 \\
 &  & highpass & 0.87 & 0.63 & 62.08 & 47.36 \\
 &  & lowpass & 0.63 & 0.31 & 36.79 & 22.07 \\
 &  & music & 0.41 & 0.08 & 21.22 & 6.50 \\
 &  & pgd & 0.44 & 0.23 & 33.87 & 19.15 \\
 &  & phaser & 0.45 & 0.11 & 23.10 & 8.38 \\
 &  & pitch down & 0.73 & 0.53 & 56.44 & 41.72 \\
 &  & pitch up & 0.66 & 0.44 & 46.73 & 32.01 \\
 &  & real rir & 0.44 & 0.19 & 29.92 & 15.20 \\
 &  & resample & 0.56 & 0.17 & 24.85 & 10.13 \\
 &  & rir & 0.33 & 0.12 & 23.86 & 9.14 \\
 &  & slowdown & 0.59 & 0.37 & 42.57 & 27.91 \\
 &  & speedup & 0.81 & 0.59 & 57.45 & 42.73 \\
 &  & tempo down & 0.23 & 0.00 & 14.85 & 0.31 \\
 &  & tempo up & 0.47 & 0.25 & 32.44 & 17.72 \\
 &  & treble & 0.43 & 0.00 & 14.86 & 0.22 \\
 &  & tremolo & 0.37 & 0.02 & 15.69 & 0.97 \\
 &  & universal adv & 0.39 & 0.02 & 15.87 & 1.17 \\
 &  & voice conversion & 0.46 & 0.16 & 22.91 & 8.19 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.63 & 0.61 & 53.17 & 51.11 \\
 &  & itw nf ami & 0.83 & 0.77 & 29.68 & 27.62 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.83 & 0.81 & 83.17 & 81.11 \\
 &  & itw nf & 0.72 & 0.70 & 56.63 & 54.58 \\
 & common voice & accent & 0.90 & 0.78 & 14.92 & 12.87 \\
\multirow[c]{77}{*}{mms-1b} & \multirow[c]{25}{*}{LibriSpeech} & clean & 1.14 & 0.00 & 15.40 & 0.00 \\
 &  & crosstalk & 0.72 & 0.31 & 32.75 & 17.34 \\
 &  & echo & 0.66 & 0.36 & 33.82 & 18.41 \\
 &  & env noise & 0.30 & 0.06 & 20.28 & 4.87 \\
 &  & env noise esc50 & 0.32 & 0.02 & 16.94 & 1.54 \\
 &  & env noise musan & 0.40 & 0.03 & 17.57 & 2.17 \\
 &  & env noise wham & 0.41 & 0.05 & 19.92 & 4.51 \\
 &  & gain & 0.29 & 0.05 & 19.13 & 3.72 \\
 &  & gnoise & 0.25 & 0.07 & 22.37 & 6.97 \\
 &  & highpass & 0.82 & 0.53 & 51.29 & 35.89 \\
 &  & lowpass & 0.55 & 0.22 & 32.51 & 17.10 \\
 &  & music & 0.41 & 0.04 & 18.23 & 2.82 \\
 &  & pgd & 0.92 & 0.62 & 59.97 & 44.56 \\
 &  & phaser & 0.67 & 0.13 & 25.00 & 9.59 \\
 &  & pitch down & 0.53 & 0.32 & 40.72 & 25.32 \\
 &  & pitch up & 0.68 & 0.43 & 42.09 & 26.69 \\
 &  & real rir & 0.48 & 0.20 & 30.99 & 15.59 \\
 &  & resample & 0.68 & 0.13 & 24.01 & 8.61 \\
 &  & rir & 0.25 & 0.02 & 16.97 & 1.62 \\
 &  & slowdown & 0.35 & 0.08 & 21.60 & 6.26 \\
 &  & speedup & 0.76 & 0.51 & 49.97 & 34.56 \\
 &  & tempo down & 0.31 & 0.01 & 15.66 & 0.32 \\
 &  & tempo up & 0.45 & 0.18 & 27.31 & 11.90 \\
 &  & universal adv & 18.14 & 6.21 & 21.65 & 6.24 \\
 &  & voice conversion & 0.49 & 0.18 & 24.27 & 8.86 \\
 & \multirow[c]{18}{*}{MLS-ES} & clean & 0.68 & 0.00 & 15.67 & 0.00 \\
 &  & echo & 1.34 & 0.76 & 36.16 & 20.49 \\
 &  & env noise & 0.56 & 0.33 & 42.28 & 26.62 \\
 &  & env noise esc50 & 1.16 & 0.35 & 28.44 & 12.77 \\
 &  & gain & 0.51 & 0.17 & 24.68 & 9.01 \\
 &  & highpass & 1.05 & 0.68 & 56.27 & 40.60 \\
 &  & lowpass & 0.50 & 0.19 & 32.40 & 16.73 \\
 &  & pgd & 1.15 & 0.86 & 69.48 & 53.82 \\
 &  & phaser & 0.88 & 0.19 & 27.28 & 11.61 \\
 &  & pitch down & 0.87 & 0.54 & 49.62 & 33.96 \\
 &  & pitch up & 1.43 & 0.93 & 49.42 & 33.76 \\
 &  & resample & 0.67 & 0.11 & 23.28 & 7.61 \\
 &  & rir & 0.64 & 0.23 & 25.06 & 9.39 \\
 &  & slowdown & 1.16 & 0.44 & 32.12 & 16.45 \\
 &  & speedup & 1.44 & 0.82 & 52.49 & 36.83 \\
 &  & tempo down & 1.30 & 0.11 & 17.47 & 1.80 \\
 &  & tempo up & 0.78 & 0.13 & 21.02 & 5.35 \\
 &  & universal adv & 0.73 & 0.20 & 23.08 & 7.41 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.99 & 0.01 & 30.80 & 0.69 \\
 &  & chorus & 0.59 & 0.10 & 36.98 & 6.75 \\
 &  & clean & 0.90 & 0.00 & 30.23 & 0.00 \\
 &  & crosstalk & 0.95 & 0.23 & 44.68 & 14.46 \\
 &  & echo & 0.74 & 0.23 & 44.00 & 13.77 \\
 &  & env noise & 0.70 & 0.06 & 35.10 & 4.88 \\
 &  & env noise esc50 & 0.68 & 0.10 & 37.75 & 7.53 \\
 &  & env noise musan & 0.66 & 0.03 & 32.46 & 2.25 \\
 &  & env noise wham & 0.69 & 0.06 & 35.19 & 4.96 \\
 &  & gain & 0.49 & 0.13 & 41.58 & 11.36 \\
 &  & gnoise & 0.43 & 0.07 & 37.51 & 7.31 \\
 &  & highpass & 0.99 & 0.50 & 67.84 & 37.61 \\
 &  & lowpass & 0.89 & 0.25 & 47.24 & 17.02 \\
 &  & music & 0.71 & 0.04 & 33.35 & 3.17 \\
 &  & pgd & 1.14 & 0.70 & 83.36 & 53.13 \\
 &  & phaser & 0.88 & 0.17 & 43.09 & 12.87 \\
 &  & pitch down & 0.76 & 0.35 & 58.04 & 27.82 \\
 &  & pitch up & 0.81 & 0.38 & 57.11 & 26.89 \\
 &  & real rir & 0.69 & 0.18 & 44.79 & 14.56 \\
 &  & resample & 0.98 & 0.17 & 40.10 & 9.88 \\
 &  & rir & 0.50 & 0.08 & 36.48 & 6.26 \\
 &  & slowdown & 0.54 & 0.09 & 36.73 & 7.11 \\
 &  & speedup & 0.92 & 0.47 & 64.21 & 33.99 \\
 &  & tempo down & 0.46 & 0.00 & 28.88 & 0.00 \\
 &  & tempo up & 0.69 & 0.24 & 47.17 & 16.95 \\
 &  & treble & 0.89 & 0.00 & 30.39 & 0.25 \\
 &  & tremolo & 0.70 & 0.00 & 29.45 & 0.00 \\
 &  & universal adv & 0.95 & 0.00 & 29.91 & 0.00 \\
 &  & voice conversion & 0.54 & 0.00 & 27.17 & 0.00 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 1.02 & 0.84 & 85.73 & 70.33 \\
 &  & itw nf ami & 1.95 & 1.52 & 69.73 & 54.32 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 1.41 & 1.26 & 141.23 & 125.83 \\
 &  & itw nf & 1.45 & 1.25 & 113.34 & 97.94 \\
 & common voice & accent & 1.97 & 1.03 & 32.65 & 17.25 \\
\multirow[c]{59}{*}{spch-t5} & \multirow[c]{25}{*}{LibriSpeech} & clean & 0.54 & 0.00 & 7.24 & 0.00 \\
 &  & crosstalk & 3.08 & 2.88 & 147.49 & 140.25 \\
 &  & echo & 1.07 & 0.93 & 55.05 & 47.81 \\
 &  & env noise & 0.69 & 0.57 & 53.69 & 46.45 \\
 &  & env noise esc50 & 0.43 & 0.28 & 28.00 & 20.76 \\
 &  & env noise musan & 0.44 & 0.27 & 25.48 & 18.25 \\
 &  & env noise wham & 0.56 & 0.39 & 40.44 & 33.20 \\
 &  & gain & 0.21 & 0.09 & 14.02 & 6.79 \\
 &  & gnoise & 0.35 & 0.26 & 33.47 & 26.23 \\
 &  & highpass & 0.94 & 0.80 & 62.26 & 55.03 \\
 &  & lowpass & 0.73 & 0.58 & 51.57 & 44.34 \\
 &  & music & 0.73 & 0.55 & 46.87 & 39.63 \\
 &  & pgd & 1.84 & 1.70 & 113.66 & 106.43 \\
 &  & phaser & 0.40 & 0.14 & 18.11 & 10.88 \\
 &  & pitch down & 0.72 & 0.62 & 56.17 & 48.93 \\
 &  & pitch up & 0.83 & 0.71 & 51.79 & 44.56 \\
 &  & real rir & 1.24 & 1.10 & 84.38 & 77.15 \\
 &  & resample & 0.63 & 0.37 & 31.46 & 24.23 \\
 &  & rir & 1.25 & 1.14 & 85.87 & 78.64 \\
 &  & slowdown & 0.69 & 0.56 & 46.99 & 39.76 \\
 &  & speedup & 0.93 & 0.81 & 61.80 & 54.57 \\
 &  & tempo down & 0.33 & 0.19 & 17.20 & 9.97 \\
 &  & tempo up & 0.27 & 0.14 & 16.63 & 9.40 \\
 &  & universal adv & 57.97 & 52.37 & 59.55 & 52.37 \\
 &  & voice conversion & 1.46 & 1.31 & 71.54 & 64.30 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 1.30 & 0.09 & 41.30 & 4.32 \\
 &  & chorus & 0.79 & 0.22 & 50.70 & 14.63 \\
 &  & clean & 1.11 & 0.00 & 36.98 & 0.00 \\
 &  & crosstalk & 2.26 & 1.38 & 119.08 & 82.10 \\
 &  & echo & 1.32 & 0.69 & 77.89 & 40.91 \\
 &  & env noise & 1.17 & 0.39 & 67.80 & 31.01 \\
 &  & env noise esc50 & 0.89 & 0.18 & 50.83 & 13.86 \\
 &  & env noise musan & 0.94 & 0.18 & 50.27 & 13.66 \\
 &  & env noise wham & 1.04 & 0.27 & 60.93 & 24.19 \\
 &  & gain & 0.98 & 0.53 & 83.28 & 46.30 \\
 &  & gnoise & 0.56 & 0.15 & 49.85 & 15.20 \\
 &  & highpass & 1.46 & 0.86 & 101.57 & 64.59 \\
 &  & lowpass & 1.56 & 0.77 & 88.35 & 51.38 \\
 &  & music & 1.14 & 0.33 & 62.59 & 25.85 \\
 &  & pgd & 1.70 & 1.16 & 127.62 & 90.64 \\
 &  & phaser & 1.16 & 0.29 & 60.02 & 23.05 \\
 &  & pitch down & 1.16 & 0.66 & 88.40 & 51.43 \\
 &  & pitch up & 1.14 & 0.61 & 80.55 & 43.57 \\
 &  & real rir & 1.32 & 0.69 & 90.47 & 53.50 \\
 &  & resample & 1.56 & 0.57 & 69.80 & 32.83 \\
 &  & rir & 1.19 & 0.67 & 86.82 & 49.85 \\
 &  & slowdown & 1.00 & 0.45 & 69.61 & 32.99 \\
 &  & speedup & 1.64 & 1.10 & 115.78 & 78.81 \\
 &  & tempo down & 0.58 & 0.03 & 37.39 & 2.41 \\
 &  & tempo up & 1.18 & 0.63 & 81.01 & 44.03 \\
 &  & treble & 1.03 & 0.00 & 35.48 & 0.00 \\
 &  & tremolo & 1.02 & 0.13 & 44.77 & 7.79 \\
 &  & universal adv & 1.39 & 0.45 & 68.75 & 31.78 \\
 &  & voice conversion & 1.17 & 0.43 & 58.64 & 21.66 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 3.72 & 3.63 & 311.57 & 304.34 \\
 &  & itw nf ami & 6.41 & 6.20 & 229.15 & 221.92 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 5.35 & 5.27 & 534.92 & 527.69 \\
 &  & itw nf & 5.07 & 4.98 & 395.97 & 388.73 \\
 & common voice & accent & 5.96 & 5.52 & 96.98 & 89.74 \\
\multirow[c]{63}{*}{w2v2-bs} & \multirow[c]{29}{*}{LibriSpeech} & bass & 0.26 & 0.10 & 8.08 & 4.35 \\
 &  & chorus & 0.36 & 0.29 & 21.16 & 17.43 \\
 &  & clean & 0.28 & 0.00 & 3.73 & 0.00 \\
 &  & crosstalk & 0.66 & 0.56 & 34.21 & 30.48 \\
 &  & echo & 1.00 & 0.93 & 51.77 & 48.04 \\
 &  & env noise & 0.26 & 0.20 & 20.53 & 16.80 \\
 &  & env noise esc50 & 0.44 & 0.37 & 28.91 & 25.18 \\
 &  & env noise musan & 0.23 & 0.14 & 13.85 & 10.12 \\
 &  & env noise wham & 0.31 & 0.22 & 22.37 & 18.64 \\
 &  & gain & 0.25 & 0.20 & 17.92 & 14.19 \\
 &  & gnoise & 0.41 & 0.37 & 40.16 & 36.43 \\
 &  & highpass & 0.81 & 0.74 & 53.12 & 49.39 \\
 &  & lowpass & 0.56 & 0.48 & 36.88 & 33.15 \\
 &  & music & 0.26 & 0.17 & 16.01 & 12.28 \\
 &  & pgd & 0.87 & 0.80 & 57.28 & 53.55 \\
 &  & phaser & 0.28 & 0.15 & 14.14 & 10.41 \\
 &  & pitch down & 0.62 & 0.57 & 48.45 & 44.72 \\
 &  & pitch up & 0.83 & 0.77 & 51.79 & 48.06 \\
 &  & real rir & 0.41 & 0.34 & 29.13 & 25.40 \\
 &  & resample & 0.54 & 0.41 & 29.41 & 25.68 \\
 &  & rir & 0.16 & 0.10 & 11.04 & 7.31 \\
 &  & slowdown & 0.54 & 0.48 & 37.44 & 33.72 \\
 &  & speedup & 0.82 & 0.76 & 54.20 & 50.47 \\
 &  & tempo down & 0.12 & 0.04 & 5.94 & 2.21 \\
 &  & tempo up & 0.20 & 0.14 & 12.66 & 8.93 \\
 &  & treble & 0.22 & 0.02 & 4.41 & 0.68 \\
 &  & tremolo & 0.16 & 0.03 & 5.63 & 1.90 \\
 &  & universal adv & 32.25 & 29.36 & 33.18 & 29.45 \\
 &  & voice conversion & 0.27 & 0.20 & 13.35 & 9.62 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.68 & 0.06 & 22.24 & 3.44 \\
 &  & chorus & 0.65 & 0.35 & 42.03 & 23.23 \\
 &  & clean & 0.56 & 0.00 & 18.80 & 0.00 \\
 &  & crosstalk & 0.86 & 0.41 & 44.48 & 25.68 \\
 &  & echo & 1.07 & 0.75 & 63.36 & 44.56 \\
 &  & env noise & 0.58 & 0.19 & 33.71 & 14.91 \\
 &  & env noise esc50 & 0.66 & 0.30 & 38.34 & 19.54 \\
 &  & env noise musan & 0.54 & 0.14 & 29.45 & 10.65 \\
 &  & env noise wham & 0.58 & 0.19 & 35.88 & 17.08 \\
 &  & gain & 0.60 & 0.38 & 51.74 & 32.94 \\
 &  & gnoise & 0.53 & 0.30 & 48.79 & 29.99 \\
 &  & highpass & 1.00 & 0.70 & 69.22 & 50.42 \\
 &  & lowpass & 1.00 & 0.60 & 54.17 & 35.37 \\
 &  & music & 0.56 & 0.15 & 30.18 & 11.42 \\
 &  & pgd & 0.51 & 0.24 & 38.74 & 19.94 \\
 &  & phaser & 0.74 & 0.30 & 38.12 & 19.32 \\
 &  & pitch down & 0.90 & 0.64 & 68.50 & 49.70 \\
 &  & pitch up & 0.90 & 0.63 & 63.39 & 44.59 \\
 &  & real rir & 0.66 & 0.35 & 45.24 & 26.44 \\
 &  & resample & 1.05 & 0.55 & 48.18 & 29.37 \\
 &  & rir & 0.62 & 0.36 & 45.61 & 26.81 \\
 &  & slowdown & 0.76 & 0.48 & 53.64 & 34.84 \\
 &  & speedup & 0.96 & 0.68 & 67.48 & 48.68 \\
 &  & tempo down & 0.36 & 0.06 & 22.60 & 3.80 \\
 &  & tempo up & 0.58 & 0.29 & 39.41 & 20.61 \\
 &  & treble & 0.57 & 0.02 & 19.83 & 1.05 \\
 &  & tremolo & 0.54 & 0.09 & 25.49 & 6.69 \\
 &  & universal adv & 0.60 & 0.12 & 25.93 & 7.13 \\
 &  & voice conversion & 0.56 & 0.19 & 28.26 & 9.46 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.83 & 0.79 & 69.71 & 65.98 \\
 &  & itw nf ami & 1.02 & 0.92 & 36.58 & 32.85 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.92 & 0.89 & 92.42 & 88.69 \\
 &  & itw nf & 0.87 & 0.83 & 68.35 & 64.62 \\
 & common voice & accent & 1.74 & 1.52 & 29.11 & 25.38 \\
\multirow[c]{27}{*}{w2v2-bs-es} & \multirow[c]{27}{*}{MLS-ES} & bass & 1.24 & 0.36 & 38.30 & 12.58 \\
 &  & chorus & 2.03 & 1.10 & 62.61 & 36.89 \\
 &  & clean & 1.12 & 0.00 & 25.72 & 0.00 \\
 &  & crosstalk & 2.14 & 0.91 & 49.76 & 24.04 \\
 &  & echo & 2.71 & 1.76 & 73.43 & 47.71 \\
 &  & env noise & 0.80 & 0.42 & 58.26 & 32.54 \\
 &  & env noise esc50 & 2.20 & 0.88 & 50.69 & 24.98 \\
 &  & env noise musan & 1.12 & 0.22 & 37.30 & 11.58 \\
 &  & env noise wham & 1.10 & 0.20 & 41.53 & 15.82 \\
 &  & gain & 0.93 & 0.38 & 47.01 & 21.29 \\
 &  & gnoise & 0.69 & 0.26 & 49.91 & 24.20 \\
 &  & highpass & 1.66 & 1.04 & 78.16 & 52.44 \\
 &  & lowpass & 1.01 & 0.50 & 58.96 & 33.25 \\
 &  & music & 0.95 & 0.21 & 39.14 & 13.42 \\
 &  & pgd & 1.00 & 0.53 & 59.51 & 33.79 \\
 &  & phaser & 1.53 & 0.39 & 45.81 & 20.09 \\
 &  & pitch down & 1.26 & 0.72 & 68.30 & 42.58 \\
 &  & pitch up & 2.27 & 1.46 & 75.77 & 50.05 \\
 &  & resample & 1.30 & 0.39 & 48.17 & 22.45 \\
 &  & rir & 1.08 & 0.41 & 42.78 & 17.07 \\
 &  & slowdown & 1.87 & 0.69 & 57.67 & 31.95 \\
 &  & speedup & 2.31 & 1.30 & 74.09 & 48.37 \\
 &  & tempo down & 2.20 & 0.24 & 30.01 & 4.29 \\
 &  & tempo up & 1.34 & 0.27 & 35.67 & 9.95 \\
 &  & treble & 1.87 & 0.09 & 28.53 & 2.82 \\
 &  & tremolo & 1.05 & 0.11 & 31.00 & 5.28 \\
 &  & universal adv & 1.07 & 0.21 & 35.72 & 10.00 \\
\multirow[c]{63}{*}{w2v2-lg} & \multirow[c]{29}{*}{LibriSpeech} & bass & 0.17 & 0.04 & 5.07 & 2.14 \\
 &  & chorus & 0.30 & 0.24 & 17.34 & 14.35 \\
 &  & clean & 0.22 & 0.00 & 2.99 & 0.00 \\
 &  & crosstalk & 0.57 & 0.49 & 30.12 & 27.13 \\
 &  & echo & 0.87 & 0.81 & 44.75 & 41.75 \\
 &  & env noise & 0.19 & 0.14 & 15.17 & 12.18 \\
 &  & env noise esc50 & 0.34 & 0.28 & 22.63 & 19.63 \\
 &  & env noise musan & 0.16 & 0.09 & 9.30 & 6.30 \\
 &  & env noise wham & 0.22 & 0.15 & 15.74 & 12.75 \\
 &  & gain & 0.13 & 0.08 & 9.00 & 6.01 \\
 &  & gnoise & 0.32 & 0.28 & 31.15 & 28.15 \\
 &  & highpass & 0.71 & 0.65 & 47.48 & 44.49 \\
 &  & lowpass & 0.45 & 0.39 & 31.60 & 28.60 \\
 &  & music & 0.18 & 0.11 & 11.48 & 8.49 \\
 &  & pgd & 0.67 & 0.61 & 47.27 & 44.27 \\
 &  & phaser & 0.21 & 0.10 & 10.66 & 7.66 \\
 &  & pitch down & 0.51 & 0.47 & 40.49 & 37.49 \\
 &  & pitch up & 0.64 & 0.59 & 40.15 & 37.16 \\
 &  & real rir & 0.32 & 0.26 & 22.89 & 19.90 \\
 &  & resample & 0.41 & 0.30 & 22.64 & 19.64 \\
 &  & rir & 0.10 & 0.05 & 6.72 & 3.72 \\
 &  & slowdown & 0.42 & 0.37 & 30.11 & 27.12 \\
 &  & speedup & 0.65 & 0.60 & 43.99 & 41.00 \\
 &  & tempo down & 0.07 & 0.02 & 3.83 & 0.83 \\
 &  & tempo up & 0.14 & 0.08 & 8.57 & 5.58 \\
 &  & treble & 0.15 & 0.00 & 2.92 & 0.03 \\
 &  & tremolo & 0.11 & 0.00 & 3.23 & 0.26 \\
 &  & universal adv & 31.28 & 28.97 & 32.02 & 29.02 \\
 &  & voice conversion & 0.24 & 0.17 & 11.59 & 8.60 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.57 & 0.04 & 18.44 & 1.93 \\
 &  & chorus & 0.59 & 0.32 & 37.73 & 21.22 \\
 &  & clean & 0.49 & 0.00 & 16.50 & 0.00 \\
 &  & crosstalk & 0.78 & 0.39 & 40.76 & 24.26 \\
 &  & echo & 0.92 & 0.64 & 54.34 & 37.84 \\
 &  & env noise & 0.50 & 0.15 & 28.71 & 12.21 \\
 &  & env noise esc50 & 0.47 & 0.15 & 27.78 & 11.27 \\
 &  & env noise musan & 0.45 & 0.10 & 23.94 & 7.44 \\
 &  & env noise wham & 0.49 & 0.15 & 29.77 & 13.27 \\
 &  & gain & 0.48 & 0.28 & 41.14 & 24.63 \\
 &  & gnoise & 0.44 & 0.25 & 41.20 & 24.70 \\
 &  & highpass & 0.90 & 0.63 & 63.51 & 47.01 \\
 &  & lowpass & 0.82 & 0.47 & 46.50 & 30.00 \\
 &  & music & 0.48 & 0.11 & 25.36 & 8.86 \\
 &  & pgd & 0.45 & 0.21 & 34.36 & 17.86 \\
 &  & phaser & 0.58 & 0.19 & 31.02 & 14.52 \\
 &  & pitch down & 0.76 & 0.53 & 58.42 & 41.91 \\
 &  & pitch up & 0.74 & 0.50 & 52.67 & 36.17 \\
 &  & real rir & 0.56 & 0.28 & 38.53 & 22.03 \\
 &  & resample & 0.83 & 0.39 & 39.52 & 23.02 \\
 &  & rir & 0.45 & 0.22 & 33.21 & 16.71 \\
 &  & slowdown & 0.64 & 0.40 & 45.94 & 29.46 \\
 &  & speedup & 0.82 & 0.58 & 58.38 & 41.87 \\
 &  & tempo down & 0.27 & 0.01 & 17.48 & 1.00 \\
 &  & tempo up & 0.46 & 0.22 & 32.02 & 15.51 \\
 &  & treble & 0.49 & 0.01 & 16.99 & 0.51 \\
 &  & tremolo & 0.44 & 0.05 & 19.66 & 3.15 \\
 &  & universal adv & 0.49 & 0.07 & 20.66 & 4.16 \\
 &  & voice conversion & 0.51 & 0.18 & 25.72 & 9.22 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.75 & 0.71 & 62.58 & 59.59 \\
 &  & itw nf ami & 0.94 & 0.86 & 33.79 & 30.80 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.90 & 0.87 & 89.93 & 86.94 \\
 &  & itw nf & 0.83 & 0.79 & 64.65 & 61.66 \\
 & common voice & accent & 1.38 & 1.20 & 23.01 & 20.02 \\
\multirow[c]{27}{*}{w2v2-lg-es} & \multirow[c]{27}{*}{MLS-ES} & bass & 0.51 & 0.27 & 15.71 & 8.88 \\
 &  & chorus & 0.93 & 0.69 & 32.16 & 25.33 \\
 &  & clean & 0.30 & 0.00 & 6.82 & 0.00 \\
 &  & crosstalk & 1.15 & 0.83 & 29.42 & 22.59 \\
 &  & echo & 2.00 & 1.75 & 54.07 & 47.25 \\
 &  & env noise & 0.42 & 0.33 & 34.03 & 27.20 \\
 &  & env noise esc50 & 0.80 & 0.45 & 23.55 & 16.73 \\
 &  & env noise musan & 0.32 & 0.09 & 12.09 & 5.31 \\
 &  & env noise wham & 0.33 & 0.10 & 16.05 & 9.37 \\
 &  & gain & 0.35 & 0.20 & 17.83 & 11.01 \\
 &  & gnoise & 0.32 & 0.21 & 28.79 & 22.07 \\
 &  & highpass & 0.96 & 0.80 & 54.95 & 48.12 \\
 &  & lowpass & 0.35 & 0.21 & 25.97 & 19.14 \\
 &  & music & 0.30 & 0.10 & 13.98 & 7.17 \\
 &  & pgd & 1.28 & 1.16 & 77.86 & 71.04 \\
 &  & phaser & 0.46 & 0.16 & 16.66 & 9.84 \\
 &  & pitch down & 0.76 & 0.62 & 47.43 & 40.61 \\
 &  & pitch up & 1.26 & 1.04 & 45.15 & 38.32 \\
 &  & resample & 0.34 & 0.10 & 13.32 & 6.50 \\
 &  & rir & 0.30 & 0.13 & 12.13 & 5.31 \\
 &  & slowdown & 0.87 & 0.56 & 36.76 & 29.93 \\
 &  & speedup & 1.31 & 1.05 & 53.39 & 46.57 \\
 &  & tempo down & 0.62 & 0.10 & 8.63 & 1.80 \\
 &  & tempo up & 0.45 & 0.16 & 13.57 & 6.75 \\
 &  & treble & 0.46 & 0.00 & 6.70 & 0.00 \\
 &  & tremolo & 0.26 & 0.01 & 7.49 & 0.67 \\
 &  & universal adv & 0.93 & 0.70 & 40.61 & 33.86 \\
\multirow[c]{63}{*}{w2v2-lg-rob} & \multirow[c]{29}{*}{LibriSpeech} & bass & 0.15 & 0.03 & 4.30 & 1.66 \\
 &  & chorus & 0.24 & 0.19 & 13.87 & 11.24 \\
 &  & clean & 0.20 & 0.00 & 2.63 & 0.00 \\
 &  & crosstalk & 0.52 & 0.45 & 28.11 & 25.48 \\
 &  & echo & 0.75 & 0.70 & 38.71 & 36.08 \\
 &  & env noise & 0.14 & 0.09 & 10.70 & 8.06 \\
 &  & env noise esc50 & 0.23 & 0.17 & 15.38 & 12.75 \\
 &  & env noise musan & 0.11 & 0.05 & 6.29 & 3.66 \\
 &  & env noise wham & 0.13 & 0.07 & 8.93 & 6.30 \\
 &  & gain & 0.08 & 0.04 & 5.86 & 3.23 \\
 &  & gnoise & 0.18 & 0.15 & 17.72 & 15.09 \\
 &  & highpass & 0.66 & 0.61 & 45.06 & 42.43 \\
 &  & lowpass & 0.28 & 0.22 & 20.12 & 17.49 \\
 &  & music & 0.12 & 0.06 & 7.31 & 4.68 \\
 &  & pgd & 0.94 & 0.89 & 63.61 & 60.98 \\
 &  & phaser & 0.16 & 0.07 & 7.64 & 5.01 \\
 &  & pitch down & 0.56 & 0.52 & 44.50 & 41.87 \\
 &  & pitch up & 0.56 & 0.52 & 35.01 & 32.37 \\
 &  & real rir & 0.22 & 0.17 & 15.63 & 12.99 \\
 &  & resample & 0.24 & 0.14 & 11.94 & 9.31 \\
 &  & rir & 0.06 & 0.02 & 4.21 & 1.58 \\
 &  & slowdown & 0.43 & 0.39 & 30.55 & 27.92 \\
 &  & speedup & 0.64 & 0.59 & 43.26 & 40.63 \\
 &  & tempo down & 0.06 & 0.01 & 2.93 & 0.29 \\
 &  & tempo up & 0.18 & 0.13 & 11.24 & 8.60 \\
 &  & treble & 0.14 & 0.00 & 2.73 & 0.09 \\
 &  & tremolo & 0.10 & 0.01 & 2.88 & 0.24 \\
 &  & universal adv & 47.82 & 45.78 & 48.43 & 45.80 \\
 &  & voice conversion & 0.17 & 0.12 & 8.56 & 5.92 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.51 & 0.02 & 16.22 & 1.04 \\
 &  & chorus & 0.47 & 0.23 & 30.55 & 15.36 \\
 &  & clean & 0.45 & 0.00 & 15.19 & 0.00 \\
 &  & crosstalk & 0.71 & 0.35 & 37.48 & 22.29 \\
 &  & echo & 0.80 & 0.55 & 47.50 & 32.31 \\
 &  & env noise & 0.43 & 0.11 & 24.28 & 9.09 \\
 &  & env noise esc50 & 0.33 & 0.04 & 18.25 & 3.06 \\
 &  & env noise musan & 0.38 & 0.06 & 19.73 & 4.55 \\
 &  & env noise wham & 0.40 & 0.08 & 22.90 & 7.71 \\
 &  & gain & 0.40 & 0.22 & 34.50 & 19.31 \\
 &  & gnoise & 0.34 & 0.15 & 30.92 & 15.73 \\
 &  & highpass & 0.82 & 0.58 & 59.17 & 43.99 \\
 &  & lowpass & 0.62 & 0.29 & 35.86 & 20.67 \\
 &  & music & 0.41 & 0.07 & 20.72 & 5.53 \\
 &  & pgd & 0.43 & 0.22 & 33.05 & 17.86 \\
 &  & phaser & 0.51 & 0.16 & 27.74 & 12.55 \\
 &  & pitch down & 0.77 & 0.57 & 59.87 & 44.68 \\
 &  & pitch up & 0.69 & 0.47 & 48.98 & 33.80 \\
 &  & real rir & 0.46 & 0.21 & 31.25 & 16.06 \\
 &  & resample & 0.63 & 0.23 & 28.92 & 13.73 \\
 &  & rir & 0.34 & 0.13 & 25.11 & 9.93 \\
 &  & slowdown & 0.63 & 0.41 & 45.30 & 30.15 \\
 &  & speedup & 0.87 & 0.64 & 61.49 & 46.30 \\
 &  & tempo down & 0.24 & 0.01 & 15.58 & 0.50 \\
 &  & tempo up & 0.51 & 0.29 & 35.45 & 20.26 \\
 &  & treble & 0.45 & 0.00 & 15.32 & 0.19 \\
 &  & tremolo & 0.38 & 0.02 & 16.39 & 1.20 \\
 &  & universal adv & 0.40 & 0.02 & 16.19 & 1.00 \\
 &  & voice conversion & 0.49 & 0.18 & 24.43 & 9.24 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.64 & 0.61 & 53.74 & 51.10 \\
 &  & itw nf ami & 0.76 & 0.69 & 27.31 & 24.67 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.86 & 0.83 & 85.99 & 83.36 \\
 &  & itw nf & 0.70 & 0.67 & 54.93 & 52.30 \\
 & common voice & accent & 1.00 & 0.84 & 16.58 & 13.94 \\
\multirow[c]{63}{*}{w2v2-lg-slf} & \multirow[c]{29}{*}{LibriSpeech} & bass & 0.11 & 0.03 & 3.37 & 1.55 \\
 &  & chorus & 0.14 & 0.11 & 8.34 & 6.51 \\
 &  & clean & 0.14 & 0.00 & 1.82 & 0.00 \\
 &  & crosstalk & 0.42 & 0.37 & 22.64 & 20.82 \\
 &  & echo & 0.61 & 0.58 & 31.28 & 29.46 \\
 &  & env noise & 0.11 & 0.08 & 8.91 & 7.09 \\
 &  & env noise esc50 & 0.21 & 0.18 & 15.01 & 13.19 \\
 &  & env noise musan & 0.09 & 0.05 & 5.59 & 3.78 \\
 &  & env noise wham & 0.11 & 0.07 & 8.00 & 6.18 \\
 &  & gain & 0.07 & 0.04 & 4.84 & 3.02 \\
 &  & gnoise & 0.19 & 0.17 & 18.92 & 17.09 \\
 &  & highpass & 0.59 & 0.55 & 40.30 & 38.48 \\
 &  & lowpass & 0.29 & 0.25 & 21.37 & 19.55 \\
 &  & music & 0.10 & 0.06 & 6.26 & 4.44 \\
 &  & pgd & 0.91 & 0.88 & 59.78 & 57.96 \\
 &  & phaser & 0.14 & 0.07 & 7.38 & 5.55 \\
 &  & pitch down & 0.49 & 0.46 & 38.81 & 36.99 \\
 &  & pitch up & 0.42 & 0.39 & 26.13 & 24.30 \\
 &  & real rir & 0.20 & 0.16 & 14.37 & 12.55 \\
 &  & resample & 0.16 & 0.10 & 8.32 & 6.50 \\
 &  & rir & 0.04 & 0.02 & 2.95 & 1.13 \\
 &  & slowdown & 0.34 & 0.31 & 24.56 & 22.73 \\
 &  & speedup & 0.52 & 0.49 & 35.83 & 34.01 \\
 &  & tempo down & 0.04 & 0.00 & 1.95 & 0.13 \\
 &  & tempo up & 0.10 & 0.07 & 6.16 & 4.34 \\
 &  & treble & 0.10 & 0.00 & 1.85 & 0.04 \\
 &  & tremolo & 0.07 & 0.00 & 2.00 & 0.18 \\
 &  & universal adv & 13.95 & 12.54 & 14.36 & 12.54 \\
 &  & voice conversion & 0.15 & 0.11 & 7.29 & 5.47 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.46 & 0.02 & 14.73 & 1.24 \\
 &  & chorus & 0.40 & 0.19 & 25.81 & 12.31 \\
 &  & clean & 0.40 & 0.00 & 13.50 & 0.00 \\
 &  & crosstalk & 0.62 & 0.30 & 32.33 & 18.84 \\
 &  & echo & 0.68 & 0.45 & 40.11 & 26.62 \\
 &  & env noise & 0.39 & 0.11 & 22.41 & 8.91 \\
 &  & env noise esc50 & 0.39 & 0.13 & 22.06 & 8.56 \\
 &  & env noise musan & 0.36 & 0.07 & 18.89 & 5.39 \\
 &  & env noise wham & 0.38 & 0.10 & 22.29 & 8.79 \\
 &  & gain & 0.44 & 0.28 & 37.81 & 24.32 \\
 &  & gnoise & 0.35 & 0.19 & 32.78 & 19.29 \\
 &  & highpass & 0.81 & 0.60 & 58.63 & 45.14 \\
 &  & lowpass & 0.64 & 0.35 & 37.51 & 24.01 \\
 &  & music & 0.38 & 0.08 & 19.72 & 6.23 \\
 &  & pgd & 0.48 & 0.29 & 37.48 & 23.98 \\
 &  & phaser & 0.50 & 0.18 & 27.60 & 14.10 \\
 &  & pitch down & 0.73 & 0.54 & 56.25 & 42.76 \\
 &  & pitch up & 0.64 & 0.45 & 45.55 & 32.06 \\
 &  & real rir & 0.44 & 0.21 & 30.02 & 16.53 \\
 &  & resample & 0.69 & 0.33 & 30.31 & 16.81 \\
 &  & rir & 0.37 & 0.18 & 26.64 & 13.15 \\
 &  & slowdown & 0.58 & 0.38 & 41.49 & 27.99 \\
 &  & speedup & 0.77 & 0.57 & 54.58 & 41.08 \\
 &  & tempo down & 0.22 & 0.01 & 14.11 & 0.61 \\
 &  & tempo up & 0.41 & 0.21 & 28.52 & 15.02 \\
 &  & treble & 0.41 & 0.01 & 14.00 & 0.51 \\
 &  & tremolo & 0.35 & 0.03 & 15.45 & 1.95 \\
 &  & universal adv & 0.37 & 0.03 & 15.04 & 1.55 \\
 &  & voice conversion & 0.47 & 0.20 & 23.36 & 9.86 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.63 & 0.60 & 52.43 & 50.60 \\
 &  & itw nf ami & 0.78 & 0.73 & 27.97 & 26.15 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.83 & 0.82 & 83.42 & 81.59 \\
 &  & itw nf & 0.69 & 0.67 & 53.80 & 51.98 \\
 & common voice & accent & 0.92 & 0.81 & 15.36 & 13.54 \\
\multirow[c]{86}{*}{wsp-bs} & \multirow[c]{25}{*}{LibriSpeech} & clean & 0.44 & 0.00 & 5.87 & 0.00 \\
 &  & crosstalk & 0.48 & 0.32 & 24.38 & 18.51 \\
 &  & echo & 0.56 & 0.44 & 28.32 & 22.45 \\
 &  & env noise & 0.18 & 0.08 & 12.98 & 7.11 \\
 &  & env noise esc50 & 0.14 & 0.03 & 7.93 & 2.06 \\
 &  & env noise musan & 0.19 & 0.05 & 9.16 & 3.29 \\
 &  & env noise wham & 0.20 & 0.06 & 11.34 & 5.47 \\
 &  & gain & 0.16 & 0.07 & 10.64 & 4.77 \\
 &  & gnoise & 0.18 & 0.11 & 16.83 & 10.96 \\
 &  & highpass & 2.80 & 2.69 & 193.78 & 187.91 \\
 &  & lowpass & 0.71 & 0.59 & 51.26 & 45.39 \\
 &  & music & 0.18 & 0.04 & 9.09 & 3.22 \\
 &  & pgd & 1.60 & 1.48 & 102.58 & 96.71 \\
 &  & phaser & 0.40 & 0.19 & 20.09 & 14.22 \\
 &  & pitch down & 0.65 & 0.57 & 52.30 & 46.43 \\
 &  & pitch up & 0.28 & 0.19 & 17.57 & 11.70 \\
 &  & real rir & 0.28 & 0.17 & 19.14 & 13.27 \\
 &  & resample & 0.47 & 0.26 & 22.39 & 16.52 \\
 &  & rir & 0.19 & 0.11 & 13.61 & 7.74 \\
 &  & slowdown & 0.70 & 0.60 & 50.83 & 44.96 \\
 &  & speedup & 0.47 & 0.37 & 31.54 & 25.67 \\
 &  & tempo down & 0.16 & 0.05 & 8.44 & 2.57 \\
 &  & tempo up & 0.16 & 0.06 & 9.88 & 4.01 \\
 &  & universal adv & 8.18 & 3.63 & 9.51 & 3.64 \\
 &  & voice conversion & 0.29 & 0.17 & 14.38 & 8.51 \\
 & \multirow[c]{27}{*}{MLS-ES} & bass & 0.86 & 0.35 & 27.52 & 12.67 \\
 &  & chorus & 1.00 & 0.47 & 30.73 & 15.88 \\
 &  & clean & 0.65 & 0.00 & 14.85 & 0.00 \\
 &  & crosstalk & 2.20 & 1.49 & 56.84 & 42.00 \\
 &  & echo & 1.58 & 1.03 & 42.58 & 27.73 \\
 &  & env noise & 0.88 & 0.67 & 73.37 & 58.52 \\
 &  & env noise esc50 & 0.89 & 0.13 & 20.32 & 5.47 \\
 &  & env noise musan & 0.64 & 0.13 & 22.17 & 7.34 \\
 &  & env noise wham & 0.69 & 0.18 & 30.64 & 15.79 \\
 &  & gain & 0.68 & 0.36 & 33.06 & 18.21 \\
 &  & gnoise & 0.51 & 0.26 & 42.14 & 27.29 \\
 &  & highpass & 4.19 & 3.83 & 253.14 & 238.29 \\
 &  & lowpass & 1.20 & 0.90 & 96.11 & 81.26 \\
 &  & music & 0.53 & 0.11 & 22.17 & 7.38 \\
 &  & pgd & 2.90 & 2.63 & 174.32 & 159.47 \\
 &  & phaser & 1.10 & 0.45 & 43.69 & 28.84 \\
 &  & pitch down & 1.81 & 1.50 & 121.50 & 106.66 \\
 &  & pitch up & 1.32 & 0.85 & 46.16 & 31.31 \\
 &  & resample & 0.91 & 0.39 & 40.86 & 26.01 \\
 &  & rir & 0.58 & 0.19 & 23.02 & 8.17 \\
 &  & slowdown & 2.09 & 1.41 & 97.43 & 82.61 \\
 &  & speedup & 1.83 & 1.25 & 75.18 & 60.33 \\
 &  & tempo down & 1.38 & 0.25 & 19.98 & 5.13 \\
 &  & tempo up & 0.88 & 0.27 & 24.36 & 9.51 \\
 &  & treble & 1.02 & 0.01 & 15.25 & 0.55 \\
 &  & tremolo & 0.63 & 0.09 & 19.05 & 4.20 \\
 &  & universal adv & 0.88 & 0.39 & 34.22 & 19.45 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.47 & 0.03 & 15.16 & 1.82 \\
 &  & chorus & 0.30 & 0.08 & 18.80 & 5.47 \\
 &  & clean & 0.40 & 0.00 & 13.33 & 0.00 \\
 &  & crosstalk & 0.60 & 0.29 & 31.96 & 18.62 \\
 &  & echo & 0.38 & 0.16 & 22.41 & 9.08 \\
 &  & env noise & 0.35 & 0.07 & 18.90 & 5.56 \\
 &  & env noise esc50 & 0.28 & 0.03 & 15.54 & 2.21 \\
 &  & env noise musan & 0.31 & 0.03 & 15.76 & 2.43 \\
 &  & env noise wham & 0.32 & 0.04 & 17.17 & 3.84 \\
 &  & gain & 0.29 & 0.13 & 24.61 & 11.28 \\
 &  & gnoise & 0.25 & 0.09 & 22.14 & 8.81 \\
 &  & highpass & 2.72 & 2.50 & 207.26 & 193.93 \\
 &  & lowpass & 0.94 & 0.66 & 60.43 & 47.09 \\
 &  & music & 0.32 & 0.02 & 15.18 & 1.86 \\
 &  & pgd & 1.23 & 1.04 & 93.62 & 80.29 \\
 &  & phaser & 0.56 & 0.25 & 33.38 & 20.04 \\
 &  & pitch down & 1.07 & 0.89 & 85.61 & 72.27 \\
 &  & pitch up & 0.38 & 0.18 & 26.60 & 13.26 \\
 &  & real rir & 0.37 & 0.15 & 25.48 & 12.15 \\
 &  & resample & 0.66 & 0.30 & 31.58 & 18.25 \\
 &  & rir & 0.25 & 0.06 & 18.15 & 4.82 \\
 &  & slowdown & 1.04 & 0.84 & 77.95 & 64.61 \\
 &  & speedup & 0.56 & 0.36 & 40.04 & 26.70 \\
 &  & tempo down & 0.22 & 0.01 & 14.30 & 0.96 \\
 &  & tempo up & 0.26 & 0.06 & 17.79 & 4.46 \\
 &  & treble & 0.40 & 0.01 & 13.68 & 0.34 \\
 &  & tremolo & 0.34 & 0.02 & 14.79 & 1.46 \\
 &  & universal adv & 0.36 & 0.02 & 15.06 & 1.74 \\
 &  & voice conversion & 0.35 & 0.08 & 17.42 & 4.09 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.54 & 0.47 & 45.41 & 39.54 \\
 &  & itw nf ami & 0.70 & 0.53 & 24.94 & 19.07 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.89 & 0.83 & 89.26 & 83.39 \\
 &  & itw nf & 0.53 & 0.45 & 41.38 & 35.51 \\
 & common voice & accent & 0.94 & 0.58 & 15.83 & 9.96 \\
\multirow[c]{16}{*}{wsp-bs.en} & \multirow[c]{16}{*}{LibriSpeech} & clean & 0.38 & 0.00 & 5.12 & 0.00 \\
 &  & echo & 0.50 & 0.40 & 25.30 & 20.18 \\
 &  & env noise esc50 & 0.27 & 0.17 & 17.50 & 12.38 \\
 &  & gain & 0.13 & 0.05 & 8.80 & 3.68 \\
 &  & highpass & 2.06 & 1.97 & 142.16 & 137.05 \\
 &  & lowpass & 0.62 & 0.51 & 44.72 & 39.60 \\
 &  & phaser & 0.32 & 0.14 & 15.42 & 10.30 \\
 &  & pitch down & 0.57 & 0.50 & 45.98 & 40.86 \\
 &  & pitch up & 0.26 & 0.18 & 16.06 & 10.95 \\
 &  & resample & 0.36 & 0.18 & 16.59 & 11.48 \\
 &  & rir & 0.11 & 0.03 & 7.26 & 2.14 \\
 &  & slowdown & 0.50 & 0.41 & 35.51 & 30.39 \\
 &  & speedup & 0.48 & 0.40 & 32.82 & 27.71 \\
 &  & tempo down & 0.14 & 0.04 & 7.31 & 2.20 \\
 &  & tempo up & 0.13 & 0.04 & 7.84 & 2.72 \\
 &  & voice conversion & 0.27 & 0.16 & 13.20 & 8.08 \\
\multirow[c]{90}{*}{wsp-lg} & \multirow[c]{29}{*}{LibriSpeech} & bass & 0.19 & 0.03 & 5.19 & 1.55 \\
 &  & chorus & 0.08 & 0.01 & 4.51 & 0.62 \\
 &  & clean & 0.29 & 0.00 & 3.89 & 0.00 \\
 &  & crosstalk & 0.18 & 0.08 & 8.63 & 4.81 \\
 &  & echo & 0.09 & 0.02 & 4.71 & 0.82 \\
 &  & env noise & 0.08 & 0.02 & 5.62 & 2.01 \\
 &  & env noise esc50 & 0.11 & 0.04 & 7.08 & 3.34 \\
 &  & env noise musan & 0.10 & 0.01 & 4.27 & 0.53 \\
 &  & env noise wham & 0.10 & 0.01 & 4.92 & 1.22 \\
 &  & gain & 0.06 & 0.01 & 4.19 & 0.39 \\
 &  & gnoise & 0.08 & 0.03 & 7.27 & 3.47 \\
 &  & highpass & 0.32 & 0.25 & 21.83 & 17.94 \\
 &  & lowpass & 0.17 & 0.09 & 10.81 & 6.99 \\
 &  & music & 0.09 & 0.00 & 3.93 & 0.39 \\
 &  & pgd & 0.68 & 0.61 & 47.52 & 43.63 \\
 &  & phaser & 0.16 & 0.03 & 5.95 & 2.15 \\
 &  & pitch down & 0.11 & 0.05 & 8.35 & 4.48 \\
 &  & pitch up & 0.07 & 0.01 & 4.53 & 0.76 \\
 &  & real rir & 0.17 & 0.10 & 12.02 & 8.27 \\
 &  & resample & 0.16 & 0.03 & 5.96 & 2.26 \\
 &  & rir & 0.06 & 0.00 & 3.84 & 0.04 \\
 &  & slowdown & 0.13 & 0.06 & 8.54 & 4.65 \\
 &  & speedup & 0.08 & 0.02 & 5.09 & 1.27 \\
 &  & tempo down & 0.11 & 0.04 & 5.79 & 1.90 \\
 &  & tempo up & 0.07 & 0.00 & 3.94 & 0.16 \\
 &  & treble & 0.19 & 0.00 & 3.62 & 0.00 \\
 &  & tremolo & 0.12 & 0.00 & 3.43 & 0.00 \\
 &  & universal adv & 6.38 & 3.37 & 7.28 & 3.39 \\
 &  & voice conversion & 0.16 & 0.08 & 7.89 & 4.00 \\
 & \multirow[c]{27}{*}{MLS-ES} & bass & 0.45 & 0.25 & 13.81 & 8.03 \\
 &  & chorus & 0.26 & 0.05 & 7.60 & 1.82 \\
 &  & clean & 0.25 & 0.00 & 5.78 & 0.00 \\
 &  & crosstalk & 0.50 & 0.23 & 12.14 & 6.39 \\
 &  & echo & 0.27 & 0.05 & 7.24 & 1.46 \\
 &  & env noise & 0.32 & 0.23 & 26.98 & 21.20 \\
 &  & env noise esc50 & 0.52 & 0.22 & 15.67 & 9.89 \\
 &  & env noise musan & 0.23 & 0.02 & 7.27 & 1.51 \\
 &  & env noise wham & 0.24 & 0.04 & 9.81 & 4.07 \\
 &  & gain & 0.28 & 0.16 & 14.80 & 9.03 \\
 &  & gnoise & 0.15 & 0.06 & 11.64 & 5.89 \\
 &  & highpass & 0.63 & 0.49 & 40.39 & 34.61 \\
 &  & lowpass & 0.22 & 0.11 & 15.51 & 9.73 \\
 &  & music & 0.19 & 0.02 & 7.18 & 1.43 \\
 &  & pgd & 1.08 & 0.97 & 70.82 & 65.04 \\
 &  & phaser & 0.32 & 0.07 & 10.15 & 4.38 \\
 &  & pitch down & 0.24 & 0.12 & 14.52 & 8.74 \\
 &  & pitch up & 0.23 & 0.04 & 7.33 & 1.55 \\
 &  & resample & 0.24 & 0.04 & 8.58 & 2.84 \\
 &  & rir & 0.21 & 0.06 & 8.37 & 2.59 \\
 &  & slowdown & 0.41 & 0.15 & 14.49 & 8.82 \\
 &  & speedup & 0.36 & 0.13 & 10.85 & 5.07 \\
 &  & tempo down & 0.61 & 0.18 & 9.76 & 4.05 \\
 &  & tempo up & 0.30 & 0.06 & 7.45 & 1.67 \\
 &  & treble & 0.40 & 0.00 & 5.73 & 0.00 \\
 &  & tremolo & 0.21 & 0.00 & 5.91 & 0.14 \\
 &  & universal adv & 0.46 & 0.27 & 19.45 & 13.67 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.40 & 0.01 & 12.42 & 0.33 \\
 &  & chorus & 0.22 & 0.02 & 13.61 & 1.48 \\
 &  & clean & 0.36 & 0.00 & 12.13 & 0.00 \\
 &  & crosstalk & 0.37 & 0.08 & 17.47 & 5.34 \\
 &  & echo & 0.24 & 0.03 & 13.94 & 1.81 \\
 &  & env noise & 0.28 & 0.03 & 14.25 & 2.13 \\
 &  & env noise esc50 & 0.29 & 0.06 & 16.95 & 4.82 \\
 &  & env noise musan & 0.26 & 0.01 & 12.80 & 0.67 \\
 &  & env noise wham & 0.27 & 0.01 & 13.42 & 1.31 \\
 &  & gain & 0.18 & 0.03 & 14.80 & 2.67 \\
 &  & gnoise & 0.17 & 0.03 & 14.71 & 2.58 \\
 &  & highpass & 0.68 & 0.48 & 50.04 & 37.91 \\
 &  & lowpass & 0.35 & 0.09 & 18.92 & 6.80 \\
 &  & music & 0.27 & 0.01 & 12.56 & 0.49 \\
 &  & pgd & 0.98 & 0.80 & 75.78 & 63.65 \\
 &  & phaser & 0.32 & 0.04 & 14.98 & 2.85 \\
 &  & pitch down & 0.26 & 0.09 & 19.89 & 7.75 \\
 &  & pitch up & 0.21 & 0.04 & 14.68 & 2.55 \\
 &  & real rir & 0.32 & 0.11 & 21.45 & 9.32 \\
 &  & resample & 0.37 & 0.05 & 14.86 & 2.79 \\
 &  & rir & 0.18 & 0.01 & 13.10 & 0.97 \\
 &  & slowdown & 0.22 & 0.04 & 15.04 & 2.91 \\
 &  & speedup & 0.21 & 0.03 & 14.31 & 2.18 \\
 &  & tempo down & 0.20 & 0.01 & 12.81 & 0.68 \\
 &  & tempo up & 0.20 & 0.02 & 13.47 & 1.34 \\
 &  & treble & 0.42 & 0.07 & 14.35 & 2.22 \\
 &  & tremolo & 0.30 & 0.01 & 12.81 & 0.68 \\
 &  & universal adv & 0.43 & 0.12 & 21.11 & 9.00 \\
 &  & voice conversion & 0.25 & 0.01 & 12.54 & 0.41 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.40 & 0.35 & 33.21 & 29.32 \\
 &  & itw nf ami & 0.55 & 0.44 & 19.80 & 15.91 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.52 & 0.49 & 52.51 & 48.62 \\
 &  & itw nf & 0.33 & 0.28 & 25.48 & 21.59 \\
 & common voice & accent & 0.46 & 0.22 & 7.58 & 3.69 \\
\multirow[c]{59}{*}{wsp-md} & \multirow[c]{25}{*}{LibriSpeech} & clean & 0.29 & 0.00 & 3.85 & 0.00 \\
 &  & crosstalk & 0.17 & 0.07 & 7.86 & 4.07 \\
 &  & echo & 0.11 & 0.03 & 5.59 & 1.74 \\
 &  & env noise & 0.09 & 0.03 & 6.13 & 2.33 \\
 &  & env noise esc50 & 0.14 & 0.07 & 8.93 & 5.08 \\
 &  & env noise musan & 0.10 & 0.01 & 4.60 & 0.80 \\
 &  & env noise wham & 0.11 & 0.02 & 5.60 & 1.75 \\
 &  & gain & 0.07 & 0.01 & 4.80 & 0.95 \\
 &  & gnoise & 0.08 & 0.03 & 7.08 & 3.25 \\
 &  & highpass & 0.87 & 0.80 & 61.25 & 57.46 \\
 &  & lowpass & 0.25 & 0.17 & 17.24 & 13.40 \\
 &  & music & 0.10 & 0.01 & 4.41 & 0.62 \\
 &  & pgd & 0.81 & 0.74 & 55.75 & 51.90 \\
 &  & phaser & 0.16 & 0.03 & 6.07 & 2.23 \\
 &  & pitch down & 0.14 & 0.09 & 11.09 & 7.24 \\
 &  & pitch up & 0.08 & 0.01 & 4.70 & 0.85 \\
 &  & real rir & 0.18 & 0.11 & 13.04 & 9.25 \\
 &  & resample & 0.20 & 0.07 & 8.36 & 4.57 \\
 &  & rir & 0.06 & 0.00 & 4.20 & 0.35 \\
 &  & slowdown & 0.14 & 0.08 & 9.49 & 5.64 \\
 &  & speedup & 0.10 & 0.03 & 6.15 & 2.32 \\
 &  & tempo down & 0.11 & 0.04 & 5.84 & 1.99 \\
 &  & tempo up & 0.08 & 0.01 & 4.45 & 0.61 \\
 &  & universal adv & 4.68 & 1.71 & 5.53 & 1.71 \\
 &  & voice conversion & 0.19 & 0.11 & 9.11 & 5.26 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.40 & 0.01 & 12.38 & 0.39 \\
 &  & chorus & 0.21 & 0.02 & 13.00 & 0.98 \\
 &  & clean & 0.36 & 0.00 & 12.02 & 0.00 \\
 &  & crosstalk & 0.36 & 0.07 & 16.65 & 4.65 \\
 &  & echo & 0.23 & 0.03 & 13.66 & 1.64 \\
 &  & env noise & 0.28 & 0.03 & 14.16 & 2.14 \\
 &  & env noise esc50 & 0.24 & 0.01 & 12.80 & 0.79 \\
 &  & env noise musan & 0.26 & 0.01 & 12.87 & 0.85 \\
 &  & env noise wham & 0.27 & 0.02 & 13.41 & 1.43 \\
 &  & gain & 0.18 & 0.04 & 15.32 & 3.30 \\
 &  & gnoise & 0.18 & 0.03 & 15.49 & 3.47 \\
 &  & highpass & 1.06 & 0.87 & 80.04 & 68.01 \\
 &  & lowpass & 0.45 & 0.19 & 25.87 & 13.84 \\
 &  & music & 0.27 & 0.01 & 12.44 & 0.46 \\
 &  & pgd & 0.91 & 0.74 & 73.28 & 61.26 \\
 &  & phaser & 0.34 & 0.06 & 16.65 & 4.63 \\
 &  & pitch down & 0.32 & 0.15 & 24.65 & 12.63 \\
 &  & pitch up & 0.21 & 0.04 & 14.62 & 2.60 \\
 &  & real rir & 0.32 & 0.12 & 22.19 & 10.17 \\
 &  & resample & 0.43 & 0.11 & 18.64 & 6.64 \\
 &  & rir & 0.18 & 0.02 & 13.22 & 1.19 \\
 &  & slowdown & 0.25 & 0.07 & 17.74 & 5.72 \\
 &  & speedup & 0.23 & 0.06 & 16.15 & 4.13 \\
 &  & tempo down & 0.20 & 0.01 & 12.50 & 0.51 \\
 &  & tempo up & 0.21 & 0.03 & 13.99 & 1.97 \\
 &  & treble & 0.37 & 0.01 & 12.64 & 0.62 \\
 &  & tremolo & 0.29 & 0.01 & 12.32 & 0.30 \\
 &  & universal adv & 0.38 & 0.08 & 17.72 & 5.70 \\
 &  & voice conversion & 0.26 & 0.02 & 12.86 & 0.84 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.39 & 0.35 & 33.07 & 29.21 \\
 &  & itw nf ami & 0.55 & 0.44 & 19.70 & 15.85 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.54 & 0.51 & 54.42 & 50.57 \\
 &  & itw nf & 0.34 & 0.29 & 26.64 & 22.79 \\
 & common voice & accent & 0.48 & 0.25 & 7.94 & 4.09 \\
\multirow[c]{16}{*}{wsp-md.en} & \multirow[c]{16}{*}{LibriSpeech} & clean & 0.31 & 0.00 & 4.13 & 0.00 \\
 &  & echo & 0.11 & 0.03 & 5.47 & 1.35 \\
 &  & env noise esc50 & 0.14 & 0.06 & 8.98 & 4.90 \\
 &  & gain & 0.07 & 0.01 & 4.84 & 0.73 \\
 &  & highpass & 0.73 & 0.65 & 49.83 & 45.79 \\
 &  & lowpass & 0.25 & 0.17 & 17.34 & 13.27 \\
 &  & phaser & 0.18 & 0.04 & 6.87 & 2.80 \\
 &  & pitch down & 0.12 & 0.06 & 9.09 & 4.99 \\
 &  & pitch up & 0.09 & 0.02 & 5.42 & 1.29 \\
 &  & resample & 0.20 & 0.07 & 8.30 & 4.34 \\
 &  & rir & 0.07 & 0.01 & 4.58 & 0.46 \\
 &  & slowdown & 0.13 & 0.06 & 8.36 & 4.28 \\
 &  & speedup & 0.12 & 0.05 & 7.84 & 3.79 \\
 &  & tempo down & 0.11 & 0.03 & 5.63 & 1.51 \\
 &  & tempo up & 0.08 & 0.01 & 4.68 & 0.60 \\
 &  & voice conversion & 0.18 & 0.10 & 8.91 & 4.79 \\
\multirow[c]{59}{*}{wsp-sm} & \multirow[c]{25}{*}{LibriSpeech} & clean & 0.32 & 0.00 & 4.27 & 0.00 \\
 &  & crosstalk & 0.24 & 0.13 & 11.59 & 7.32 \\
 &  & echo & 0.22 & 0.14 & 11.33 & 7.06 \\
 &  & env noise & 0.11 & 0.04 & 7.72 & 3.45 \\
 &  & env noise esc50 & 0.19 & 0.10 & 12.06 & 7.79 \\
 &  & env noise musan & 0.12 & 0.02 & 5.68 & 1.42 \\
 &  & env noise wham & 0.13 & 0.03 & 7.02 & 2.76 \\
 &  & gain & 0.09 & 0.02 & 5.96 & 1.69 \\
 &  & gnoise & 0.10 & 0.05 & 9.67 & 5.40 \\
 &  & highpass & 1.22 & 1.14 & 85.65 & 81.38 \\
 &  & lowpass & 0.37 & 0.28 & 25.78 & 21.51 \\
 &  & music & 0.12 & 0.01 & 5.38 & 1.11 \\
 &  & pgd & 1.20 & 1.12 & 75.39 & 71.11 \\
 &  & phaser & 0.21 & 0.06 & 8.88 & 4.61 \\
 &  & pitch down & 0.26 & 0.20 & 20.40 & 16.13 \\
 &  & pitch up & 0.12 & 0.05 & 7.17 & 2.90 \\
 &  & real rir & 0.22 & 0.14 & 15.75 & 11.48 \\
 &  & resample & 0.26 & 0.11 & 11.34 & 7.08 \\
 &  & rir & 0.08 & 0.02 & 5.36 & 1.09 \\
 &  & slowdown & 0.22 & 0.15 & 15.25 & 10.98 \\
 &  & speedup & 0.16 & 0.09 & 10.22 & 5.95 \\
 &  & tempo down & 0.12 & 0.04 & 6.32 & 2.05 \\
 &  & tempo up & 0.10 & 0.03 & 6.10 & 1.83 \\
 &  & universal adv & 11.56 & 8.25 & 12.52 & 8.25 \\
 &  & voice conversion & 0.23 & 0.14 & 11.23 & 6.96 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.41 & 0.01 & 12.98 & 0.67 \\
 &  & chorus & 0.22 & 0.03 & 14.06 & 1.75 \\
 &  & clean & 0.37 & 0.00 & 12.31 & 0.00 \\
 &  & crosstalk & 0.39 & 0.10 & 18.86 & 6.54 \\
 &  & echo & 0.26 & 0.06 & 15.69 & 3.37 \\
 &  & env noise & 0.29 & 0.03 & 15.06 & 2.75 \\
 &  & env noise esc50 & 0.25 & 0.01 & 13.13 & 0.81 \\
 &  & env noise musan & 0.27 & 0.02 & 13.45 & 1.14 \\
 &  & env noise wham & 0.28 & 0.02 & 14.27 & 1.96 \\
 &  & gain & 0.20 & 0.05 & 16.64 & 4.33 \\
 &  & gnoise & 0.20 & 0.05 & 17.24 & 4.93 \\
 &  & highpass & 1.43 & 1.23 & 109.80 & 97.49 \\
 &  & lowpass & 0.53 & 0.26 & 31.41 & 19.09 \\
 &  & music & 0.28 & 0.01 & 13.15 & 0.87 \\
 &  & pgd & 1.06 & 0.88 & 82.12 & 69.80 \\
 &  & phaser & 0.38 & 0.09 & 19.19 & 6.88 \\
 &  & pitch down & 0.47 & 0.30 & 37.26 & 24.95 \\
 &  & pitch up & 0.23 & 0.05 & 16.08 & 3.76 \\
 &  & real rir & 0.34 & 0.13 & 23.23 & 10.91 \\
 &  & resample & 0.45 & 0.12 & 19.50 & 7.19 \\
 &  & rir & 0.20 & 0.03 & 14.69 & 2.38 \\
 &  & slowdown & 0.42 & 0.23 & 30.08 & 17.77 \\
 &  & speedup & 0.28 & 0.10 & 19.39 & 7.07 \\
 &  & tempo down & 0.20 & 0.01 & 12.87 & 0.56 \\
 &  & tempo up & 0.23 & 0.04 & 15.15 & 2.83 \\
 &  & treble & 0.37 & 0.01 & 12.66 & 0.35 \\
 &  & tremolo & 0.31 & 0.02 & 13.01 & 0.69 \\
 &  & universal adv & 0.34 & 0.03 & 14.55 & 2.24 \\
 &  & voice conversion & 0.28 & 0.03 & 13.94 & 1.62 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.42 & 0.37 & 35.63 & 31.36 \\
 &  & itw nf ami & 0.59 & 0.47 & 21.23 & 16.96 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.63 & 0.59 & 63.46 & 59.19 \\
 &  & itw nf & 0.37 & 0.32 & 29.19 & 24.92 \\
 & common voice & accent & 0.65 & 0.39 & 10.77 & 6.50 \\
\multirow[c]{16}{*}{wsp-sm.en} & \multirow[c]{16}{*}{LibriSpeech} & clean & 0.30 & 0.00 & 4.04 & 0.00 \\
 &  & echo & 0.21 & 0.14 & 10.92 & 6.88 \\
 &  & env noise esc50 & 0.17 & 0.09 & 10.94 & 6.91 \\
 &  & gain & 0.09 & 0.02 & 5.81 & 1.77 \\
 &  & highpass & 1.63 & 1.55 & 116.22 & 112.19 \\
 &  & lowpass & 0.33 & 0.25 & 23.10 & 19.07 \\
 &  & phaser & 0.20 & 0.06 & 8.36 & 4.33 \\
 &  & pitch down & 0.22 & 0.16 & 17.11 & 13.07 \\
 &  & pitch up & 0.13 & 0.06 & 7.84 & 3.80 \\
 &  & resample & 0.25 & 0.10 & 10.77 & 6.74 \\
 &  & rir & 0.07 & 0.01 & 4.99 & 0.95 \\
 &  & slowdown & 0.19 & 0.12 & 13.05 & 9.01 \\
 &  & speedup & 0.19 & 0.12 & 12.38 & 8.34 \\
 &  & tempo down & 0.11 & 0.03 & 5.91 & 1.87 \\
 &  & tempo up & 0.09 & 0.02 & 5.32 & 1.29 \\
 &  & voice conversion & 0.21 & 0.13 & 10.29 & 6.25 \\
\multirow[c]{85}{*}{wsp-tn} & \multirow[c]{24}{*}{LibriSpeech} & clean & 0.61 & 0.00 & 8.20 & 0.00 \\
 &  & crosstalk & 0.74 & 0.52 & 38.16 & 29.96 \\
 &  & echo & 1.00 & 0.84 & 50.92 & 42.72 \\
 &  & env noise & 0.27 & 0.14 & 19.93 & 11.73 \\
 &  & env noise esc50 & 0.47 & 0.31 & 30.85 & 22.65 \\
 &  & env noise musan & 0.28 & 0.09 & 14.15 & 5.95 \\
 &  & env noise wham & 0.29 & 0.10 & 16.33 & 8.13 \\
 &  & gain & 0.24 & 0.11 & 16.31 & 8.10 \\
 &  & gnoise & 0.27 & 0.17 & 25.61 & 17.41 \\
 &  & highpass & 2.42 & 2.27 & 157.67 & 149.47 \\
 &  & lowpass & 1.25 & 1.08 & 91.08 & 82.88 \\
 &  & music & 0.25 & 0.06 & 12.52 & 4.33 \\
 &  & phaser & 0.61 & 0.32 & 30.32 & 22.12 \\
 &  & pitch down & 1.12 & 1.01 & 90.05 & 81.85 \\
 &  & pitch up & 0.57 & 0.44 & 35.45 & 27.25 \\
 &  & real rir & 0.38 & 0.23 & 25.84 & 17.64 \\
 &  & resample & 0.81 & 0.52 & 41.40 & 33.19 \\
 &  & rir & 0.19 & 0.07 & 13.17 & 4.97 \\
 &  & slowdown & 1.14 & 1.00 & 81.73 & 73.53 \\
 &  & speedup & 0.85 & 0.72 & 57.75 & 49.55 \\
 &  & tempo down & 0.22 & 0.05 & 11.11 & 2.91 \\
 &  & tempo up & 0.25 & 0.11 & 15.40 & 7.20 \\
 &  & universal adv & 28.82 & 22.47 & 30.70 & 22.50 \\
 &  & voice conversion & 0.37 & 0.20 & 18.09 & 9.89 \\
 & \multirow[c]{27}{*}{MLS-ES} & bass & 1.71 & 0.91 & 53.01 & 29.69 \\
 &  & chorus & 1.67 & 0.83 & 51.88 & 28.56 \\
 &  & clean & 1.02 & 0.00 & 23.32 & 0.00 \\
 &  & crosstalk & 4.29 & 3.17 & 112.28 & 88.97 \\
 &  & echo & 3.29 & 2.43 & 88.87 & 65.55 \\
 &  & env noise & 1.35 & 1.01 & 109.82 & 86.50 \\
 &  & env noise esc50 & 2.44 & 1.24 & 72.18 & 48.86 \\
 &  & env noise musan & 1.03 & 0.22 & 36.46 & 13.19 \\
 &  & env noise wham & 1.04 & 0.23 & 43.62 & 20.30 \\
 &  & gain & 1.16 & 0.66 & 58.47 & 35.15 \\
 &  & gnoise & 0.89 & 0.50 & 75.64 & 52.32 \\
 &  & highpass & 4.98 & 4.42 & 261.98 & 238.66 \\
 &  & lowpass & 2.11 & 1.65 & 171.48 & 148.16 \\
 &  & music & 0.84 & 0.17 & 35.24 & 11.94 \\
 &  & pgd & 4.96 & 4.53 & 293.21 & 269.89 \\
 &  & phaser & 2.10 & 1.08 & 93.64 & 70.32 \\
 &  & pitch down & 2.85 & 2.36 & 188.14 & 164.82 \\
 &  & pitch up & 2.96 & 2.22 & 105.21 & 81.89 \\
 &  & resample & 1.94 & 1.11 & 98.71 & 75.39 \\
 &  & rir & 1.03 & 0.43 & 41.39 & 18.07 \\
 &  & slowdown & 3.23 & 2.15 & 144.75 & 121.43 \\
 &  & speedup & 3.18 & 2.26 & 132.37 & 109.05 \\
 &  & tempo down & 2.06 & 0.28 & 28.99 & 5.67 \\
 &  & tempo up & 1.35 & 0.38 & 37.91 & 14.59 \\
 &  & treble & 1.67 & 0.06 & 24.81 & 1.49 \\
 &  & tremolo & 0.99 & 0.15 & 32.47 & 9.15 \\
 &  & universal adv & 1.61 & 0.83 & 66.37 & 43.06 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.51 & 0.04 & 16.71 & 2.28 \\
 &  & chorus & 0.42 & 0.19 & 26.86 & 12.43 \\
 &  & clean & 0.43 & 0.00 & 14.44 & 0.00 \\
 &  & crosstalk & 0.72 & 0.37 & 38.58 & 24.14 \\
 &  & echo & 0.63 & 0.39 & 37.34 & 22.90 \\
 &  & env noise & 0.45 & 0.15 & 26.35 & 11.91 \\
 &  & env noise esc50 & 0.50 & 0.22 & 31.97 & 17.54 \\
 &  & env noise musan & 0.37 & 0.07 & 19.40 & 4.97 \\
 &  & env noise wham & 0.38 & 0.08 & 21.23 & 6.80 \\
 &  & gain & 0.37 & 0.20 & 31.83 & 17.40 \\
 &  & gnoise & 0.33 & 0.16 & 30.24 & 15.81 \\
 &  & highpass & 1.75 & 1.51 & 124.14 & 109.70 \\
 &  & lowpass & 1.29 & 0.98 & 83.36 & 68.92 \\
 &  & music & 0.37 & 0.05 & 18.24 & 3.80 \\
 &  & pgd & 1.73 & 1.52 & 125.33 & 110.89 \\
 &  & phaser & 0.72 & 0.38 & 44.46 & 30.02 \\
 &  & pitch down & 1.33 & 1.14 & 105.98 & 91.55 \\
 &  & pitch up & 0.64 & 0.43 & 45.18 & 30.74 \\
 &  & real rir & 0.45 & 0.20 & 30.76 & 16.33 \\
 &  & resample & 1.09 & 0.70 & 57.19 & 42.75 \\
 &  & rir & 0.33 & 0.13 & 23.94 & 9.50 \\
 &  & slowdown & 1.38 & 1.16 & 102.47 & 88.04 \\
 &  & speedup & 0.98 & 0.77 & 71.30 & 56.87 \\
 &  & tempo down & 0.25 & 0.03 & 16.21 & 1.77 \\
 &  & tempo up & 0.34 & 0.12 & 23.34 & 8.91 \\
 &  & treble & 0.44 & 0.02 & 15.46 & 1.02 \\
 &  & tremolo & 0.43 & 0.08 & 19.88 & 5.45 \\
 &  & universal adv & 0.39 & 0.02 & 15.76 & 1.32 \\
 &  & voice conversion & 0.37 & 0.09 & 18.74 & 4.31 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.68 & 0.58 & 57.12 & 48.92 \\
 &  & itw nf ami & 0.82 & 0.59 & 29.37 & 21.17 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 1.07 & 0.98 & 106.77 & 98.57 \\
 &  & itw nf & 0.70 & 0.59 & 54.47 & 46.27 \\
 & common voice & accent & 1.33 & 0.83 & 22.12 & 13.92 \\
\multirow[c]{63}{*}{wsp-tn.en} & \multirow[c]{29}{*}{LibriSpeech} & bass & 0.39 & 0.11 & 11.48 & 5.05 \\
 &  & chorus & 0.29 & 0.18 & 16.64 & 10.20 \\
 &  & clean & 0.48 & 0.00 & 6.43 & 0.00 \\
 &  & crosstalk & 0.58 & 0.41 & 30.12 & 23.68 \\
 &  & echo & 0.64 & 0.51 & 32.36 & 25.92 \\
 &  & env noise & 0.21 & 0.11 & 15.43 & 9.00 \\
 &  & env noise esc50 & 0.17 & 0.04 & 9.74 & 3.30 \\
 &  & env noise musan & 0.22 & 0.07 & 11.38 & 4.94 \\
 &  & env noise wham & 0.23 & 0.08 & 13.20 & 6.77 \\
 &  & gain & 0.19 & 0.09 & 12.99 & 6.55 \\
 &  & gnoise & 0.21 & 0.14 & 20.39 & 13.96 \\
 &  & highpass & 1.59 & 1.47 & 104.40 & 97.97 \\
 &  & lowpass & 1.45 & 1.31 & 109.77 & 103.33 \\
 &  & music & 0.21 & 0.05 & 10.32 & 3.88 \\
 &  & pgd & 1.72 & 1.60 & 96.64 & 90.21 \\
 &  & phaser & 0.44 & 0.22 & 22.09 & 15.65 \\
 &  & pitch down & 0.93 & 0.84 & 75.02 & 68.58 \\
 &  & pitch up & 0.53 & 0.42 & 32.84 & 26.41 \\
 &  & real rir & 0.32 & 0.20 & 21.69 & 15.26 \\
 &  & resample & 0.56 & 0.33 & 27.31 & 20.88 \\
 &  & rir & 0.24 & 0.14 & 16.56 & 10.13 \\
 &  & slowdown & 1.10 & 0.99 & 79.57 & 73.14 \\
 &  & speedup & 1.17 & 1.06 & 80.68 & 74.25 \\
 &  & tempo down & 0.18 & 0.05 & 9.12 & 2.69 \\
 &  & tempo up & 0.19 & 0.08 & 11.41 & 4.97 \\
 &  & treble & 0.35 & 0.01 & 7.07 & 0.63 \\
 &  & tremolo & 0.27 & 0.04 & 8.41 & 1.98 \\
 &  & universal adv & 14.39 & 9.41 & 15.86 & 9.43 \\
 &  & voice conversion & 0.32 & 0.19 & 15.63 & 9.19 \\
 & \multirow[c]{29}{*}{TEDLIUM} & bass & 0.48 & 0.03 & 15.57 & 1.90 \\
 &  & chorus & 0.34 & 0.13 & 21.87 & 8.20 \\
 &  & clean & 0.41 & 0.00 & 13.67 & 0.00 \\
 &  & crosstalk & 0.66 & 0.33 & 35.52 & 21.85 \\
 &  & echo & 0.52 & 0.29 & 30.60 & 16.93 \\
 &  & env noise & 0.38 & 0.09 & 21.25 & 7.58 \\
 &  & env noise esc50 & 0.29 & 0.03 & 15.76 & 2.09 \\
 &  & env noise musan & 0.34 & 0.05 & 17.57 & 3.90 \\
 &  & env noise wham & 0.34 & 0.06 & 18.89 & 5.22 \\
 &  & gain & 0.32 & 0.15 & 26.71 & 13.05 \\
 &  & gnoise & 0.27 & 0.11 & 24.53 & 10.87 \\
 &  & highpass & 1.22 & 1.00 & 87.75 & 74.08 \\
 &  & lowpass & 1.58 & 1.29 & 107.65 & 93.99 \\
 &  & music & 0.34 & 0.04 & 16.43 & 2.76 \\
 &  & pgd & 1.44 & 1.25 & 104.41 & 90.74 \\
 &  & phaser & 0.65 & 0.33 & 37.97 & 24.30 \\
 &  & pitch down & 1.17 & 0.99 & 93.69 & 80.02 \\
 &  & pitch up & 0.58 & 0.39 & 41.53 & 27.86 \\
 &  & real rir & 0.42 & 0.19 & 28.85 & 15.18 \\
 &  & resample & 0.73 & 0.37 & 35.97 & 22.30 \\
 &  & rir & 0.28 & 0.09 & 20.25 & 6.58 \\
 &  & slowdown & 1.28 & 1.07 & 95.37 & 81.70 \\
 &  & speedup & 1.38 & 1.18 & 101.56 & 87.89 \\
 &  & tempo down & 0.24 & 0.02 & 15.29 & 1.62 \\
 &  & tempo up & 0.29 & 0.09 & 19.76 & 6.09 \\
 &  & treble & 0.41 & 0.01 & 14.18 & 0.51 \\
 &  & tremolo & 0.37 & 0.04 & 16.32 & 2.65 \\
 &  & universal adv & 1.07 & 0.72 & 65.32 & 51.65 \\
 &  & voice conversion & 0.33 & 0.05 & 16.42 & 2.75 \\
 & \multirow[c]{2}{*}{ami} & itw ff ami & 0.57 & 0.50 & 48.10 & 41.66 \\
 &  & itw nf ami & 0.72 & 0.54 & 25.89 & 19.46 \\
 & \multirow[c]{2}{*}{chime} & itw ff & 0.87 & 0.80 & 86.88 & 80.45 \\
 &  & itw nf & 0.53 & 0.45 & 41.67 & 35.23 \\
 & common voice & accent & 1.15 & 0.75 & 19.14 & 12.70 \\
\end{tabular}

==> texfiles/table_results-by-cat-trunc-es.tex <==
\begin{tabular}{p{1.5cm}|>{\raggedleft}p{0.7cm}|>{\raggedleft}p{0.7cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.7cm}|>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.6cm}>{\raggedleft\arraybackslash}p{0.6cm}}
\toprule
 & clean & accent & audio proc & noise (env) & noise (white) & sFX & spatial & AVG & Adv (UA) & Adv (US)  & AVG \\
 & (WER) & \multicolumn{7}{c|}{(NWERD)} & \multicolumn{3}{c}{(WERD)} \\\midrule
 \midrule
cnry-1b & \textbf{3.2} & 700.7 & 21.8 & 17.4 & 7.6 & 30.5 & 36.3 & 135.7 & 26.1 & 84.3 & 55.2 \\
wsp-lg & 5.8 & \textbf{6.8} & \textbf{19.4} & \textbf{12.3} & \textbf{5.5} & \textbf{9.2} & \textbf{5.5} & \textbf{9.8} & 13.7 & 65.0 & 39.4 \\
w2v2-lg-es & 6.8 & 31.7 & 31.8 & 30.2 & 20.5 & 40.7 & 89.1 & 40.7 & 33.9 & 71.0 & 52.4 \\
wsp-bs & 14.8 & 62.1 & 133.3 & 43.1 & 25.8 & 60.5 & 58.2 & 63.8 & 19.5 & 159.5 & 89.5 \\
mms-1b & 15.7 & 7.7 & 18.5 & 19.7 & 37.1 & 20.0 & 14.9 & 19.6 & \textbf{7.4} & 53.8 & 30.6 \\
wsp-tn & 23.3 & 104.7 & 190.6 & 96.2 & 49.0 & 111.0 & 135.9 & 114.6 & 43.1 & 269.9 & 156.5 \\
w2v2-bs-es & 25.7 & 45.6 & 56.0 & 45.0 & 25.1 & 58.5 & 103.4 & 55.6 & 10.0 & \textbf{33.8} & \textbf{21.9} \\\bottomrule
\end{tabular}
